Input-to-state stability of distributed parameter systems

Input-to-state stability (ISS) allows estimating the impact of inputs and initial conditions on both the intermediate values and the asymptotic bound on the solutions. ISS has unified the input-output and Lyapunov stability theories and is a crucial property in the stability theory of control systems as well as for many applications whose dynamics depend on parameters, unknown perturbations, or other inputs. In this habilitation thesis, we provide a broad picture of infinite-dimensional input-to-state stability theory.

==> chap_ISS-linear-systems.tex <==
\section{Linear systems}
\label{sec:Linear_systems}

Having introduced the main notions of ISS theory, we proceed to systematic well-posedness and input-to-state stability analysis of evolution equations. 
In this chapter, we study well-posedness and ISS of linear systems with unbounded input operators, including linear boundary control systems.
The ISS analysis of such systems is important in particular for analyzing robustness of PDE systems w.r.t.\  boundary disturbances
as well as for robust stabilization by means of boundary controllers.
The linearity of control systems allows for efficient functional-analytic criteria for ISS, which are not available for general nonlinear systems. 
%and makes it possible to derive constructive converse Lyapunov theorems for important subclasses of linear systems.
In this chapter, we explain these methods in detail.



\subsection{Abstract linear control systems}
\label{sec:Abstract linear control systems}

We start by introducing the framework of abstract linear control systems, where we follow the approach in \cite{Wei89b} (see also \cite{TuW09}) rather closely.

Assume that $U$ and $X$ are Banach spaces, $p\in [1,\infty]$ and $\Uc:=L^p(\R_+,U)$, which is a space of strongly measurable functions $u:\R_+\to U$, such that $\|u\|_{L^p(\R_+,U)}:=\Big(\int_{\R_+}\|u(s)\|^p_U ds\Big)^{\frac{1}{p}} < \infty$.


% (see \cite[Definition 2.1]{Wei89b}).
\begin{definition}
\label{def:abstract linear control system}
\index{control system!linear abstract}
An \emph{abstract linear control system} on $X$ and $\Uc$ is a pair $(T,\Phi)$, where $T:= \sg{T} \subset L(X)$ is a strongly continuous semigroup and $\Phi:=\sg{\Phi} \subset L(\Uc,X)$ is so that for all $u,v \in\Uc$ and all $t,\tau\geq 0$ the \emph{composition property} holds:
\begin{eqnarray}
\hspace{8mm}\Phi(t+\tau)(\ccat{u}{v}{\tau}) = T(t)\Phi(\tau)u + \Phi(t)v,\quad
\ccat{u}{v}{\tau}(s):=
\begin{cases}
u(s), & \text{ if } s \in [0,\tau], \\
v(s-\tau),  & \text{ otherwise}.
\end{cases}
\label{eq:Composition-property}
\end{eqnarray}
\end{definition}
%The operators $\Phi(t)$ are also called input maps.
We immediately verify some simple properties of the family $\Phi=(\Phi(t))_{t\geq0}$:
\begin{proposition}
\label{prop:Identity-causality-growth}
Let $(T,\Phi)$ be an abstract linear control system. Then:
\begin{enumerate}[label=(\roman*)]
	\item $\Phi(0)=0$.
	\item The \emph{causality} property holds:
\[
\Phi(\tau)u = \Phi(\tau)(\ccat{u}{0}{\tau}) = \Phi(\tau)P(\tau) u,
\]
where we define the projection operator by $P(\tau) u:=\ccat{u}{0}{\tau}$, $u\in\Uc$.
		\item The map $t\mapsto \|\Phi(t)\|$ is nondecreasing.
\end{enumerate}
\end{proposition}

\begin{proof}
(i). Setting $u=v$ and $t=\tau =0$, we see that $\Phi(0)u=2\Phi(0)u$ for all $u$.

(ii). Just take $v=0$ and $t=0$.

(iii). Taking in \eqref{eq:Composition-property} $u=0$ and taking the supremum over all $v$ satisfying $\|v\|_U=1$, we get for any $t,\tau\geq 0$ that
\begin{equation*}
\|\Phi(t)\| \le \|\Phi({t+\tau})\|.
\end{equation*}
\end{proof}

The next result shows the strong continuity of the family $\Phi=(\Phi(t))_{t\geq0}$ for $p<\infty$.
\begin{proposition}
\label{prop:Wei89b-Proposition_2.3}
Let $X$ and $\Uc$ be as in Definition~\ref{def:abstract linear control system} with $p < \infty$ and
let $\Sigma=(T,\Phi)$ be an abstract linear control system
on $X$ and $\Uc$. Then the function
\begin{gather*}
q(t, u) = \Phi(t) u
\end{gather*}
is continuous on the product $\R_+ \times \Uc$. In particular, $\Phi=(\Phi(t))_{t\geq0}$ is a~strongly continuous family of operators.
\end{proposition}

\begin{proof}
Let us show the continuity of $q$ with
respect to $t$. Fix any $u\in\Uc$ and consider the map
\begin{gather*}
f_u(t):=\Phi(t) u,\quad t\geq 0.
\end{gather*}
As $t\mapsto \|\Phi(t)\|$ is nondecreasing, the causality implies for $t\in[0, 1]$ that
\begin{gather*}
\|f_u(t)\|_X = \|\Phi(t) P(t) u\|_X \le \|\Phi(1)\| \cdot \|P(t) u\|_{\Uc}.
\end{gather*}
By the dominated convergence theorem (here we use that $p<\infty$), we see that 
$\|P(t) u\|_{\Uc} \to 0$ as $t \to 0$, hence
\begin{gather*}
\lim_{t\to +0}f_u(t) = 0.
\end{gather*}
The composition property \eqref{eq:Composition-property} and strong continuity of $T$ now imply the right continuity of $f_u$.
To prove the left continuity of $f_u$ at $\tau>0$, consider a~sequence $(\varepsilon_n) \subset [0, \tau]$ such that $\varepsilon_n \to 0$ as $n\to\infty$, and define $u_n(t)=u(\varepsilon_n+t)$. 
Again invoking the dominated convergence theorem for $p<\infty$, we see that $u_n \to u$ as $n\to\infty$.

Clearly,
\begin{gather*}
u = \ccat{u}{u_n}{\varepsilon_n},
\end{gather*}
and using the composition property, we obtain that 
\begin{gather*}
\Phi({\varepsilon_n+(\tau-\varepsilon_n)})u
 = T({\tau-\varepsilon_n})\Phi({\varepsilon_n})u
 + \Phi({\tau-\varepsilon_n}) u_n.
\end{gather*}
This shows
\begin{gather*}
\Phi(\tau)u - \Phi({\tau-\varepsilon_n})u
 = T({\tau-\varepsilon_n})\Phi({\varepsilon_n})u
 + \Phi({\tau-\varepsilon_n})(u_n-u),
\end{gather*}
which yields
\begin{gather*}
\|\Phi(\tau)u - \Phi({\tau-\varepsilon_n})u\|_X
 \le M \cdot \|f_u(\varepsilon_n)\|_X + \|\Phi(\tau)\| \cdot \|u_n-u\|_{\Uc},
\end{gather*}
where $M$ is a~bound for $\|T(t)\|$ on $[0,\tau]$.
Thus, the left continuity of $f_u$ in any $\tau > 0$ is also proved.

Hence, $q$ is continuous in both arguments, and the joint continuity of $q$ follows from the decomposition
\begin{gather*}
\Phi(t) v - \Phi(\tau)u = \Phi(t)(v-u) + (\Phi(t)-\Phi(\tau))u.
\end{gather*}
\end{proof}


The next proposition shows that abstract linear control systems are a subclass of \q{general control systems}: 
%introduced in Definition~\ref{Steurungssystem}.
\begin{proposition}
\label{prop:Abstract_LCS_are_general_CS}
Let $X$, $\Uc$, $T$ and $\Phi$ be as in Definition~\ref{def:abstract linear control system}. Define
the flow map
\begin{eqnarray}
\phi(t,x,u):=T(t)x + \Phi(t)u,\quad t\geq0,\ x\in X,\ u\in\Uc.
\label{eq:Flow-map}
\end{eqnarray}
Let either $p<\infty$ or $p=\infty$ and $\phi$ be continuous w.r.t.\  time.

Then the triple $\Sigma:=(X,\Uc,\phi)$ 
 %satisfies the following properties
%\begin{sysnum}
    %\item\label{axiom:Identity} \emph{The identity property}: for every $(x,u) \in X \times \Uc$
          %it holds that $\phi(0, x,u)=x$.
    %\item \emph{Causality}: for every $(t,x,u) \in \R_+ \times X \times
          %\Uc$, for every $\tilde{u} \in \Uc$, such that $u(s) =
          %\tilde{u}(s)$ for all $s \in [0,t]$ it holds that $\phi(t,x,u) = \phi(t,x,\tilde{u})$.
    %\item \label{axiom:Continuity} \emph{Continuity}: for each $(x,u) \in X \times \Uc$ the map $t \mapsto \phi(t,x,u)$ is continuous.
  %%\item \label{axiomsyscont}
          %%Continuity with respect to initial conditions: for all $d \in
          %%\Uc, T\geq 0$ the map
          %%$\phi(\cdot,\cdot,d): X \to C([0,T],X)$, $x \mapsto
          %%\phi_{[0,T]}(\cdot,x,d)$ is continuous with respect to the
          %%supremum norm on $C([0,T],X)$.
    %%\item \label{axiom:Lipschitz} Lipschitz continuity w.r.t.\  ininital conditions on compact intervals: For any $\tau>0$ and any $R>0$ there exists $L>0$ so that for any $x,y \in X$: $\|x\|_X \leq R$, $\|y\|_X \leq R$, for all $t \in [0,\tau]$ and for all $d \in \Uc$ it holds that
%%\begin{eqnarray}
%%\|\phi(t,x,d) - \phi(t,y,d) \|_X \leq L \|x-y\|_X.
%%\label{eq:Flow_is_Lipschitz}
%%\end{eqnarray}
%%\index{semigroup property}
%%     \item Semigroup property: for all $t,h \geq 0$, for all $x \in X$, $d_1,d_2 \in \Uc$ it follows
%% $\phi(h,\phi(t,x,d_1),d_2)=\phi(t+h,x,d)$, where $d$ is defined as in \eqref{eq:Composed_Input}.
        %\item \label{axiom:Cocycle} \emph{The cocycle property}: for all $t,h \geq 0$, for all
                  %$x \in X$, $u \in \Uc$ we have
%$\phi(h,\phi(t,x,u),u(t+\cdot))=\phi(t+h,x,u)$, whenever the left or the
%right hand side of this equality is defined.
%\end{sysnum}
 is a control system in the sense of Definition~\ref{Steurungssystem}.
\end{proposition}

\begin{proof}
Clearly, the properties (i)--(iv) of Definition~\ref{Steurungssystem} are satisfied for $\Sigma$.
In view of Proposition~\ref{prop:Identity-causality-growth}, $\Phi(0)=0$, which implies the identity axiom for $\Sigma$.

Setting $t=0$ into \eqref{eq:Composition-property}, we obtain that
$\Phi(\tau)(\ccat{u}{v}{\tau}) = \Phi(\tau)u$, for any $u,v\in\Uc$, and thus for all $\tau\geq 0$, $x\in X$ and $u,v\in\Uc$,
it holds that
\[
\phi(\tau,x,\ccat{u}{v}{\tau})=T(\tau)x + \Phi(\tau)(\ccat{u}{v}{\tau}) = T(\tau)x + \Phi(\tau)u =\phi(\tau,x,u),
\]
which shows the causality property of $\Sigma$.

For $p=\infty$ we take the continuity of $\phi$ w.r.t.\  time by assumption, and for $p<\infty$ the continuity axiom follows from Proposition~\ref{prop:Wei89b-Proposition_2.3} and strong continuity of $T$.

%that $\{\Phi(t):t\geq 0\}$ is a strongly continuous family of operators, see \cite[Proposition 2.3]{Wei89b}.

Finally, the cocycle property for $\Sigma$ follows by the following computation, valid for all $t,\tau\ge 0$, $x \in X$, and all $u,v\in\Uc$.
\begin{eqnarray*}
\phi(t,\phi(\tau,x,u),v) &=& T(t)\phi(\tau,x,u) + \Phi(t)v \\
&=& T(t)(T(\tau)x + \Phi(\tau)u) + \Phi(t)v \\
&=& T(t+\tau)x + T(t)\Phi(\tau)u + \Phi(t)v \\
&=& T(t+\tau)x + \Phi(t+\tau)(\ccat{u}{v}{\tau}) \\
&=& \phi(t+\tau,x,\ccat{u}{v}{\tau}).
\end{eqnarray*}
%This shows that $\Sigma$ is a control system in the sense of Definition~\ref{Steurungssystem}.
\end{proof}

Having a growth rate of the semigroup $T$ of an abstract linear control system $(T,\Phi)$, one can also find the growth rate of $\Phi$.

\begin{proposition}
\label{prop:Proposition_2.5}
Let $X$ and $\Uc$ be as in Definition~\ref{def:abstract linear control system}, and let $(T,\Phi)$ be an abstract linear control system on $X$ and $\Uc$. 
Take $M \ge 1$ and $\omega \in\R$ such that
\begin{gather*}
\|T(t)\| \le M e^{\omega t},\qquad t\geq 0.
\end{gather*}
If $\omega>0$, there is some $L\geq0$ such that
\begin{gather*}
\|\Phi(t)\| \le L e^{\omega t},\qquad t\ge0.
\end{gather*}
If $\omega<0$, then there is $G>0$, such that $\|\Phi(t)\|\leq G$ for all $t\geq 0$.
\end{proposition}


\begin{proof}
From the composition property we get by induction for any $(u_k)_{k=1}^n\subset \Uc$ that
\begin{equation}
\Phi(n)\left( \dots \left(\ccat{u_1}{u_2}{1}\right)\ccat{}{}{2}
 \dots \ccat{}{}{n-1}u_n\right)
 = T({n-1}) \Phi(1) u_1
 + T({n-2}) \Phi(1) u_2
 + \dots
 + \Phi(1) u_n,
\label{eq:Book_2.4}
\end{equation}
and since $t\mapsto \|\Phi(t)\|$ is nondecreasing, we obtain for $t \in (n-1, n]$:
\begin{gather*}
\|\Phi(t)\| \le \|\Phi(n)\|
 \le \Big(\|T({n-1})\|+\|T({n-2})\|+\dots+\|I\|\Big)
 \cdot \|\Phi(1)\|
 \le M \frac{e^{\omega n}-1}{e^{\omega}-1}\|\Phi(1)\|,
\end{gather*}
so we can take
\begin{gather*}
L = M \frac{e^{\omega}}{e^{\omega}-1}\|\Phi(1)\|.
\end{gather*}
If $\omega<0$, the uniform boundedness of $\sg{\Phi}$ follows easily from \eqref{eq:Book_2.4}.
\end{proof}


The following proposition resolves the question of eISS of a \emph{well-defined} abstract linear control system to the question of the exponential stability of the semigroup $T$.
\begin{proposition}
\label{prop:ISS_abstract:linear:systems}
Under the assumptions of Proposition~\ref{prop:Abstract_LCS_are_general_CS}, the following statements are equivalent:
\begin{itemize}
    \item[(i)]  $\Sigma$ is eISS with a linear gain.
    %\item[(ii)] $\Sigma$ is ISS
    %\item[(iii)] $\Sigma$ is 0-UGAS
    \item[(ii)] $T$ is exponentially stable.
\end{itemize}
\end{proposition}

\begin{proof}
%We assume that $\Sigma$ is a well-defined control system. We have:
%
%\noindent(i) $\Rightarrow$ (ii) $\Rightarrow$ (iii). Clear.
\noindent(i) $\Rightarrow$ (ii). Clear.

%\noindent(ii) $\Rightarrow$ (i). 0-UGAS of $\Sigma$ means that there is $\beta \in \KL$ so that
%$\|\phi(t,x,0)\|_X = \|T(t)x\|_X \leq \beta(\|x\|_X,t)$, for all $x\in X$ and $t\geq 0$.
%In particular,
%\[
%\|T(t)\| = \sup_{\|x\|_X=1} \|T(t)x\|_X \leq \beta(1,t) \to 0,\quad t\to\infty.
%\]
%This implies that $T$ is exponentially stable, see \cite[Proposition 1.2, p. 296]{EnN00}.

\noindent(ii) $\Rightarrow$ (i). As $T$ is exponentially stable, there are $M\ge 1$, $\lambda>0$ so that $\|T(t)\|\leq M e^{-\lambda t}$ for all $t\geq 0$.
According to Proposition~\ref{prop:Proposition_2.5}, it holds that $\|\Phi(t)\|\leq G$ for a certain $G>0$ and all $t\geq 0$.
Thus, for all $t\geq0$, $x\in X$, $u\in\Uc$, we have
\begin{eqnarray*}
\|\phi(t,x,u)\|_X \leq \|T(t)x\|_X + \|\Phi(t)\| \|u\|_{\Uc}\leq Me^{-\lambda t}\|x\|_X + G \|u\|_{\Uc},
%\label{eq:ISS-estimate-abstract-linear-systems}
\end{eqnarray*}
which shows eISS of $\Sigma$ with a linear gain $G$.
\end{proof}

%\begin{theorem}{Original formulation}
%\label{thm:Representation theorem of Weiss}
%Let $U$, $X$ be Banach spaces, $p\in[0,+\infty)$ and let $\Uc:=L^p(\R_+,U)$.
%Assume that $(T,\Phi)$ be an abstract linear control system on $X$ and $\Uc$.
%Then there is a unique operator $B(U, X_{-1})$ such that for any $u$ and any $t\ge 0$
%\[
%\Phi(t)u = \int_0^t T(t-s) B u(s)ds
%\]
%Moreover, for any $x_0\in X$ and $u\in\Uc$ the function of $t\ge 0$
%\[
%\phi(t,x,u) = T(t)x  + \Phi(t)u
%\]
%is the (unique) continuous state strong solution of the differential equation
%\[
%\dot{x}(t) = A x(t) + B u(t).
%\]
%with $x(0) = x_0$
%\end{theorem}





\subsection{Representation of abstract control systems}

Assume that $X$ is a Banach space and $A:D(A)\to X$, $D(A)\subset X$ is an infinitesimal generator of a strongly continuous semigroup on $X$ (which already implies that $\rho(A) \neq \emptyset$).
Define the \emph{extrapolation space} $X_{-1}$ as the completion of $X$ with respect to the norm
$ \|x\|_{X_{-1}}:= \|(aI -A)^{-1}x\|_X$ for some $a$ in the resolvent set $\rho(A) \subset\C$ of $A$.

\begin{lemma}
\label{lem:Equivalent-norms-on-X-1} 
The space $X_{-1}$ does not depend on the choice of $a \in\rho(A)$, and different choices of $a \in \rho(A)$ generate equivalent norms on $X_{-1}$.
\end{lemma}

\begin{proof}
An easy exercise.
\ifExercises\mir{See Exercise~\ref{ex:C0_Semigroups_Ex18}.}\fi
%For any $a \in\rho(A)$ define $ \|x\|_{a}:= \|(aI -A)^{-1}x\|_X$, $x \in X$. Then we have that 
%\begin{eqnarray*}
%\|x\|_a 
%&:=& \|(aI -A)^{-1}(bI-A)(bI -A)^{-1}x\|_X \\
%&=& \|(aI -A)^{-1}(aI-A+(b-a)I)(bI -A)^{-1}x\|_X \\
%&=& \|(I+(b-a)(aI -A)^{-1})(bI -A)^{-1}x\|_X \\
%&\leq& \|I+(b-a)(aI -A)^{-1}\| \|x\|_b.
%%\label{eq:}
%\end{eqnarray*}
%Exchanging the roles of $a$ and $b$, we obtain the converse inequality.
\end{proof}

Lifting of the state space $X$ to a larger space $X_{-1}$ brings good news: the semigroup  $(T(t))_{t\ge 0}$ extends uniquely to a strongly continuous semigroup  $(T_{-1}(t))_{t\ge 0}$ on $X_{-1}$ whose generator $A_{-1}:X_{-1}\to X_{-1}$ is an extension of $A$ with $D(A_{-1}) = X$, see, e.g.,\ \cite[Section II.5]{EnN00}.


In practice, a system is usually defined by means of differential equations.
The following result shows that every abstract linear control system with $p\neq \infty$ can be represented as a flow map of a certain linear differential equation.

\begin{theorem}
\label{thm:Representation theorem of Weiss}
Let $U$, $X$ be Banach spaces, $p\in[0,+\infty)$ and let $\Uc:=L^p(\R_+,U)$.
Assume that $(T,\Phi)$ is an abstract linear control system on $X$ and $\Uc$.
Then there is a unique operator $B \in L(U, X_{-1})$ such that for any $u \in\Uc$ and any $t\ge 0$ it holds that
\begin{eqnarray}
\Phi(t)u = \int_0^t T_{-1}(t-s) B u(s)ds.
\label{eq:Phi-representation}
\end{eqnarray}
Moreover, for any $x_0\in X$ and $u\in\Uc$ the function $\phi:\R_+\times X \times \Uc \to X$, defined by
\[
\phi(t,x_0,u) = T(t)x_0  + \Phi(t)u
\]
is the (continuous) mild solution of
\[
\dot{x}(t) = A x(t) + B u(t)
\]
with $x(0) = x_0$.
\end{theorem}

According to Theorem~\ref{thm:Representation theorem of Weiss},
every abstract linear control system can be represented as a mild solution of a linear equation. However, not every pair $(A,B)$ where $A$ is a generator of a strongly continuous semigroup and $B \in L(U, X_{-1})$ gives rise to an abstract linear control system.
Theorem~\ref{thm:Representation theorem of Weiss}  tells us that (at least for $p<\infty$) the condition $B\in L(U,X_{-1})$ is a necessary (but not sufficient) condition for that.
Next, we consider the classes of input operators that do generate linear control systems. As we will see, the understanding of such classes of systems is important not only for the well-posedness theory but also for the ISS analysis of linear control systems.
The simplest class of such operators are bounded $B$ that will be discussed in the next section.
Afterwards, we turn our attention to classes of so-called admissible operators, which provide us with a much more general and wide-reaching theory.




\subsection{ISS of linear systems with bounded input operators}
\label{sec:Linear_systems_bounded_ops}

Let $X,U$ be Banach spaces. Consider a linear control system
\begin{equation}
\label{eq:Linear_System}
\dot{x}(t)=Ax(t)+ Bu(t), \quad t > 0,
\end{equation}
where $A$ is the generator of a strongly continuous semigroup $T:=(T(t))_{t\ge 0}$ on $X$ and $B\in L(U,X)$.

\ifnothabil	\sidenote{\mir{As we know from Theorem~\ref{Milde_Loesungen}}}\fi

As we know from \cite[Lemma 10.1.6]{JaZ12}, the (continuous) mild solution of \eqref{eq:Linear_System} corresponding to a certain initial condition $x_0\in X$ and to an external input $u$, is given by 
\begin{eqnarray}
\phi(t,x_0,u):=T(t)x_0 +\int_0^t T(t-s)B u(s)ds,\quad t\ge 0,
\label{eq:Lin_Sys_mild_Solution}
\end{eqnarray}
where the integral is well-defined in the sense of Bochner, see \cite[Chapter 1]{ABH11} for the Bochner integration theory.


\ifnothabil	\sidenote{\mir{see Section~\ref{sec:Bochner-integral} for the Bochner integration theory.}}\fi


Consider for $p\in[1,+\infty]$ the spaces $L^{p}_{\loc}(\R_+,W)$ of \emph{locally Bochner-integrable functions}, consisting of functions $f:\R_+\to W$ so that the restriction $f_I$ of a map $f$ to any compact interval $I \subset \R_+$ belongs to $L^p(I,W)$.

\begin{remark}
\label{rem:L_p-loc-spaces}
Note that the space $L^{1}_{\loc}(\R_+,U)$ is not a normed vector space, as some of its elements have \q{infinite} $L^1$-norm (that is, the $L^1$-norm cannot be introduced for these spaces), and hence according to Definition~\ref{Steurungssystem}, $L^{1}_{\loc}(\R_+,U)$ is not allowed as an input space to a control system. However, ISS of a control system w.r.t.\ inputs in $L^1(\R_+,U)$ implies ISS of the system with $L^{1}_{\loc}(\R_+,U)$, due to causality of the control systems, similarly to Proposition~\ref{prop:Causality_Consequence}.
Therefore, we slightly abuse the use of Definition~\ref{Steurungssystem}, and allow for the input spaces $L^{p}_{\loc}(\R_+,U)$.
\end{remark}

It is reasonable to consider ISS of \eqref{eq:Linear_System} with respect to different choices of input spaces, as defined next:
\begin{definition}
\label{def:Lp-ISS} 
Let $\Uc$ be a normed linear space of admissible inputs. 
We say that the system \eqref{eq:Linear_System} is ISS w.r.t.\  $\Uc$, if $(X,\Uc,\phi)$ with $\phi$ as in \eqref{eq:Lin_Sys_mild_Solution} is a well-posed input-to-state stable control system.

If \eqref{eq:Linear_System} is ISS w.r.t.\  $\Uc=L^p(\R_+,U)$, then we call \eqref{eq:Linear_System} $L^p$-ISS.
\end{definition}

The following lemma shows that \eqref{eq:Linear_System} is a well-posed control system with any $\Uc:=L^{p}_{\loc}(\R_+,U)$, $p\in[1,+\infty]$.
\begin{lemma}
\label{lem:Systems-with-bounded-input-operators-are-well-posed}
Consider the system \eqref{eq:Linear_System}, with $B\in L(U,X)$. Let $\Uc:=L^{p}_{\loc}(\R_+,U)$, $p\in[1,+\infty]$, and let $\Phi$ be defined by
\begin{eqnarray*}
\Phi(t)u = \int_0^t T(t-s) B u(s)ds,\quad t\geq0,\quad u\in\Uc.
%\label{eq:Phi-representation}
\end{eqnarray*}
%Then $\Sigma:=(X,\Uc,\phi)$  is a control system in the sense of Definition~\ref{Steurungssystem}.
Then $(T,\Phi)$  is a linear control system in the sense of Definition~\ref{def:abstract linear control system}.

In particular, $(T,\Phi)$ is eISS iff $T$ is exponentially stable. 
\end{lemma}

%\begin{lemma}
%\label{lem:Systems-with-bounded-input-operators-are-well-posed}
%Let $\Uc:=L^{1, loc}(\R_+,U)$, and let $\phi$ be defined by \eqref{eq:Lin_Sys_mild_Solution}.
%Then $\Sigma:=(X,\Uc,\phi)$  is a control system in the sense of Definition~\ref{Steurungssystem}.
%\end{lemma}

\begin{proof}
%For a fixed $u\in\Uc$ the map $s \mapsto T(t-s)B u(s)$ is Bochner integrable and
%$t\mapsto \int_0^t T(t-s)B u(s)ds$ is continuous, see \cite[Proposition 1.3.4]{ABH11}.\footnote{If $X$ is Hilbert space, a simpler argument can be found in \cite[Example A.1.13, Lemma 10.1.6]{JaZ12}.}
%As for a fixed $x\in X$ the map $t \mapsto T(t)x$ is continuous, $\phi$ is continuous w.r.t.\ $t$ as well.
%Verification of the other axioms of a control system is straightforward.
%Define $\Phi(t)u:=\int_0^t T(t-s)B u(s)ds$ for all $u\in\Uc$ and $t\geq 0$.
As $B$ is a bounded operator, $\Phi(t)$ is bounded for all $t\geq 0$.
Moreover,
it holds that
\begin{eqnarray*}
\Phi(t+\tau)(\ccat{u}{v}{\tau})
&=& \int_0^{t+\tau} T(t+\tau-s)B (\ccat{u}{v}{\tau})(s) ds \\
&=& \int_0^{\tau} T(t+\tau-s)B u(s) ds + \int_{\tau}^{t+\tau} T(t+\tau-s)B v(s-\tau) ds  \\
&=& T(t)\int_0^{\tau} T(\tau-s)B u(s) ds + \int_{0}^{t} T(t-s)B v(s) ds  \\
&=& T(t)\Phi(\tau)u + \Phi(t)v,
\end{eqnarray*}
which shows the composition property \eqref{eq:Composition-property} and herewith the claim of the lemma.

Application of Proposition~\ref{prop:ISS_abstract:linear:systems} finishes the proof of the lemma.
\end{proof}







\subsection{ISS of linear systems with unbounded input operators}
\label{sec:ISS of linear systems}

Assume that $X$ and $U$ are Banach spaces, $q\in [1,\infty]$, and $\Uc:=L^q(\R_+,U)$.
Let also $A:D(A) \subset X\to X$ be an infinitesimal generator of a strongly continuous semigroup $T:=(T(t))_{t\geq 0}$ on $X$ with a nonempty resolvent set $\rho(A)$.
Consider again the equation \eqref{eq:Linear_System} but now assume that $B$ is an unbounded linear operator from $U$ to $X$.
Unbounded input operators naturally appear in boundary or point control of linear systems, see, e.g., \cite{JaZ12}.

To treat this case, we again consider an extrapolation space $X_{-1}$. 
As we know from the representation Theorem~\ref{thm:Representation theorem of Weiss}, the input operator $B$ must satisfy the condition $B\in L(U,X_{-1})$ in order to give rise to a well-defined control system (at least for $q<\infty$). We assume this for all $q\in[1,\infty]$.

Thus we may consider equation \eqref{eq:Linear_System} on the Banach space $X_{-1}$:
\begin{equation}
\label{eq:Linear_System_extrapolated}
\dot{x}(t)=A_{-1}x(t)+ Bu(t), \quad t > 0,
\end{equation}
and mild solutions of this extrapolated system are given by the variation of constants formula \eqref{eq:Lin_Sys_mild_Solution}, which takes
for every $x \in X$, $u\in L^{1}_{\loc}(\R_+,U)$  and every $t\geq 0$ the form
\begin{eqnarray}
\phi(t,x,u)&:=&T_{-1}(t)x+\int_0^t T_{-1}(t-s)B u(s)ds\nonumber\\
        &=&T(t)x+\int_0^t T_{-1}(t-s)B u(s)ds.
\label{eq:Lifted_Lin_Sys_mild_Solution}
\end{eqnarray}
The last transition is due to the fact that $T_{-1}(t)x = T(t)x$ for all $x\in X$ and $t\geq 0$.

The lifting comes however at a price that now the solution $\phi(t,x,u)$ has values in $X_{-1}$.
The formula \eqref{eq:Lifted_Lin_Sys_mild_Solution} defines an $X$-valued function only provided that the value of the integral in \eqref{eq:Lifted_Lin_Sys_mild_Solution} belongs to the state space $X$, despite the fact that what we integrate is in $X_{-1}$.
This motivates the following definition:
\begin{definition}
\label{def:q-admissibility}
\index{operator!$q$-admissible}
The operator $B\in L(U,X_{-1})$ is called a {\em $q$-admissible control operator} for $(T(t))_{t\ge 0}$, where $1\le q\le \infty$, if
there is a $t>0$ so that
\begin{eqnarray}
u\in L^q(\R_+,U) \qrq \int_0^t T_{-1}(t-s)Bu(s)ds\in X.
\label{eq:q-admissibility}
\end{eqnarray}
\end{definition}
Define the operators $\Phi(t): \Uc \to X$ by
\[
\Phi(t)u := \int_0^t T_{-1}(t-s)Bu(s)ds.
\]
Note that for any $B \in L(U,X_{-1})$, the operators $\Phi(t)$ are well-defined as maps from $\Uc$ to $X_{-1}$ for all $t$. The next result shows that from $q$-admissibility of $B$ it follows that the image of $\Phi(t)$ is in $X$ for all $t \geq 0$ and with $\Uc:=L^q(\R_+,U)$ we have $\Phi(t)\in L(\Uc,X)$ for all $t>0$.

\begin{proposition}%{(\cite[Proposition 4.2]{Wei89b}, \cite[Proposition 4.2.2]{TuW09})}
\label{prop:Restatement-admissibility}
Let $X, U$ be Banach spaces and let $q \in [1,\infty]$ be given. Then $B \in L(U,X_{-1})$ is $q$-admissible for $T$ if and only if
for all $t>0$ there is $h_t>0$ so that for all $u \in L^{q}_{loc}(\R_+,U)$ it holds that $\Phi(t)u \in X$ and
%\cite{TuW09}, \cite{JaP04}, \cite{Wei89b} if
\begin{equation}
\label{eq:admissible-operator-norm-estimate}
\left\| \int_0^t T_{-1}(t-s)Bu(s)\,ds\right\|_X \le h_t \|u\|_{L^q([0,t],U)}.
\end{equation}
Furthermore, $(T,\Phi)$ defines an abstract linear control systems over $X$ and $\Uc:=L^q(\R_+,U)$.
\end{proposition}

\begin{proof}
Due to $q$-admissibility, take any $t_0$ such that \eqref{eq:q-admissibility} holds with $t:=t_0$.

Take any $\tau\in (0,t_0)$, and any $v \in L^q([0,t_0-\tau],U)$. Define $u:=\ccat{0}{v}{\tau} \in L^q([0,t_0],U)$.
Then $\Phi(t_0)u \in X$ and at the same time
\[
\Phi(t_0)u = \int_{\tau}^{t_0} T_{-1}(t_0-s)Bv(s-\tau)ds = \int_{0}^{t_0-\tau} T_{-1}(t_0 - \tau -s)Bv(s)ds = \Phi(t_0-\tau)v.
\] 
As $\tau \in (0,t_0)$ and $v \in L^q([0,t_0-\tau],U)$ are arbitrary, we see that \eqref{eq:q-admissibility} holds for all $t\in[0,t_0]$.

As in the proof of Lemma~\ref{lem:Systems-with-bounded-input-operators-are-well-posed}, one can show that for all $u_1,u_2 \in \Uc=L^q(\R_+,U)$ and all $t,\tau\geq 0$, it holds that 
\begin{eqnarray}
\Phi(\tau+t)(\ccat{u_1}{u_2}{\tau}) = T_{-1}(t)\Phi(\tau)u_1 + \Phi(t)u_2,
\label{eq:composition property-admissible-operators}
\end{eqnarray}
where the equality is considered in the space $X_{-1}$.
Now take any $t \in [0,t_0]$, and set in \eqref{eq:composition property-admissible-operators} $\tau:=t$. We have that 
\[
\Phi(2t)(\ccat{u_1}{u_2}{t}) = T_{-1}(t)\Phi(t)u_1 + \Phi(t)u_2.
\]
We have shown that $\Phi(t)u_1 \in X$. As $T_{-1}$ is an extension of $T$, we have that 
$T_{-1}(t)\Phi(t)u_1 = T(t)\Phi(t)u_1 \in X$, and thus $\Phi(2t)(\ccat{u_1}{u_2}{t}) \in X$. 
As $u_1,u_2 \in \Uc$ are arbitrary, we obtain that \eqref{eq:q-admissibility} holds for $t\in[0,2t_0]$.
Iteratively, we see that \eqref{eq:q-admissibility} holds for all $t\geq 0$.

Let us show that $\Phi(t)\in L(\Uc,X)$ for all $t>0$.

As $B\in B(U,X_{-1})$, then for $\mu \in\rho(A)$ it holds that $(\mu I - A)^{-1}B \in L(U,X)$.

\ifnothabil	\sidenote{\mir{(see Lemma~\ref{lem:Commutation_Closed_integral})}}\fi

Then, as $A$ commutes with the semigroup $T$, and using that closed operators \q{commute} with the Bochner integral
(see \cite[Proposition 1.1.7]{ABH11}), we have that 
\[
\Phi(t)u = \int_0^t T_{-1}(t-s)(\mu I - A)(\mu I - A)^{-1}Bu(s)ds 
= (\mu I - A)\int_0^t T_{-1}(t-s)(\mu I - A)^{-1}Bu(s)ds.
\]
Since $(\mu I - A)^{-1}B$ maps to $X$, and $T_{-1}$ coincides with $T$ on $X$, we have that
\[
\Phi(t)u = (\mu I - A)\int_0^t T(t-s)(\mu I - A)^{-1}Bu(s)ds.
\]
Now 
\[
u \mapsto \int_0^t T(t-s)(\mu I - A)^{-1}Bu(s)ds
\]
is a bounded operator from $\Uc$ to $X$, and thus $\Phi(t)$ is closed as a product of a closed and a bounded operator.

Since $\Phi(t)$ is defined on the whole $\Uc$, the closed graph theorem ensures that $\Phi(t) \in L(\Uc,X)$.
As $T$ and $T_{-1}$ coincide on $X$, in \eqref{eq:composition property-admissible-operators} we have that 
$T_{-1}(t)\Phi(\tau)u_1 = T(t)\Phi(\tau)u_1$ for all $t,\tau\geq 0$ and all $u_1 \in \Uc$.
Together with \eqref{eq:composition property-admissible-operators}, this shows that $(T,\Phi)$ defines an abstract linear control systems over $X$ and $\Uc$.
\end{proof}

If $B\in L(U,X_{-1})$ is a $q$-admissible operator, then $\phi$ given by \eqref{eq:Lifted_Lin_Sys_mild_Solution} is well-defined on $\R_+\times X\times \Uc$, with $\Uc:=L^q(\R_+,U)$. 
The next natural question is whether $\Sigma:=(X,\Uc,\phi)$ is a control system in the sense of Definition~\ref{Steurungssystem}.
For $q<\infty$ it has an affirmative answer:
\begin{proposition}
\label{prop:q-admissibility-implies-continuity}
Assume that $B\in L(U,X_{-1})$ is a $q$-admissible input operator with $q<\infty$.
Then $(X,\Uc,\phi)$ with $\Uc:=L^q(\R_+,U)$ and $\phi$ given by \eqref{eq:Lifted_Lin_Sys_mild_Solution} is a forward-complete control system in the sense of Definition~\ref{Steurungssystem}, satisfying the CEP and BRS properties.
\end{proposition}

\begin{proof}
Using Proposition~\ref{prop:Restatement-admissibility} and arguing as in Lemma~\ref{lem:Systems-with-bounded-input-operators-are-well-posed}, one can show that $(T,\Phi)$, where $\Phi:=\{\Phi(t):t\in\R_+\}$ is an abstract linear control system.
In view of Proposition~\ref{prop:Abstract_LCS_are_general_CS}, $(X,\Uc,\phi)$ is a control system in the sense of Definition~\ref{Steurungssystem}. CEP and BRS properties follow from the fact that $T$ is a strongly continuous semigroup and from the estimate \eqref{eq:admissible-operator-norm-estimate}.
\end{proof}

For $\infty$-admissible control operators we have the following result:
\begin{proposition}
\label{prop:infty-admissibility-implies-continuity}
Assume that $B\in L(U,X_{-1})$ is an $\infty$-admissible input operator and that $\phi$ is continuous w.r.t.\ time in the norm of $X$.
Then $(X,\Uc,\phi)$ with $\Uc:=L^\infty(\R_+,U)$ and $\phi$ given by \eqref{eq:Lifted_Lin_Sys_mild_Solution} is a forward-complete control system in the sense of Definition~\ref{Steurungssystem}, satisfying the CEP and BRS properties.
\end{proposition}

\begin{proof}
The proof resembles the proof of Proposition~\ref{prop:q-admissibility-implies-continuity}.
\end{proof}

\begin{remark}
\label{rem:Admissibility-and-forward-completeness}
In the language of general control systems, $q$-admissibility means precisely the forward-completeness of control systems for all inputs from $L^q(\R_+,U)$, which is in view of Proposition~\ref{prop:Restatement-admissibility} equivalent to BRS property.
\end{remark}

Although $\phi$ given by \eqref{eq:Lifted_Lin_Sys_mild_Solution} is continuous w.r.t.\ time in the norm of $X_{-1}$ (as a mild solution), this does not imply that $\phi$ is continuous in the $X$-norm.
The question whether $\infty$-admissibility of $B\in L(U,X_{-1})$ implies the continuity of the solution map $\phi$ w.r.t.\ time in the $X$-norm has been open for 30 years (\cite[Problem 2.4]{Wei89b}). Recently, this was positively answered in \cite{JSZ19} for an important subclass of analytic systems on Hilbert spaces:
\begin{theorem}
\label{thm:Contiuity-of-a-map}
Let $A$ generate an exponentially stable analytic semigroup on a Hilbert space $X$, which is similar to a contraction semigroup.
Assume further that $\dim (U) <\infty$.

Then any $B\in L(U,X_{-1})$ is an $\infty$-admissible operator, and the corresponding map $\phi$ is continuous in the norm of $X$ for any $u \in \Uc:=L^\infty(\R_+,U)$. Consequently, $\Sigma:=(X,\Uc,\phi)$ is a control system in the sense of Definition~\ref{Steurungssystem}.
\end{theorem}

\begin{proof}
The result follows from \cite[Theorem 1]{JSZ19}.
\end{proof}

\begin{remark}
\label{rem:Relations-between-admissibility-classes}
Lemma~\ref{prop:Restatement-admissibility} and H\"older's inequality show that $q$-admissibility of $B\in L(U,X_{-1})$ implies $p$-admissibility of $B$ for any $p>q$.
Indeed, from \eqref{eq:admissible-operator-norm-estimate} we obtain for any $p \in (q,\infty)$:
\begin{eqnarray*}
 \left\| \int_0^t T(s)Bu(s)\,ds\right\|_X &\le& h_t \Big(\int_0^t 1 \cdot |u(s)|^q ds\Big)^{1/q}\\
 &\leq &  h_t \Big(\int_0^t 1^{\frac{p}{p-q}} ds\Big)^{\frac{p-q}{p}} \Big(\int_0^t |u(s)|^p ds\Big)^{1/p}\\
 &\leq &  h_t t^{\frac{p-q}{p}} \Big(\int_0^t |u(s)|^p ds\Big)^{1/p},
\end{eqnarray*}
which is precisely $p$-admissibility of $B$. The case of $p=\infty$ is analogous.

At the same time, in general, $q$-admissibility of $B$ does not imply $p$-admissibility for any $p<q$.
In particular, in \cite[Example 5.2]{JNP18}, it was given an example of an $\infty$-admissible operator,
which is not $p$-admissible for any $p<\infty$.
Thus, admissibility gives us a measure for how bad-behaved an unbounded input operator may be, and $\infty$-admissible operators are the \q{worst} type of operators, which still allows for well-posedness of a linear control system \eqref{eq:Linear_System} and at the same time gives
the possibility to obtain ISS with respect to the supremum norm of the inputs, which is the most classical type of ISS estimates.
Bounded operators are always 1-admissible, and if $X$ is reflexive, then $1$-admissibility of $B$ is equivalent to the fact that $B\in L(U, X)$, see
\cite[Theorem 4.8]{Wei89b}.
\end{remark}



We proceed to stability analysis of linear systems with admissible input operators.
\begin{definition}
\label{def:infinite-time-admissibility}
\index{operator!infinite-time $q$-admissible}
A $q$-admissible operator $B$ is called \emph{infinite-time $q$-admissible operator}, if the constant $h:=h_t$ in Lemma~\ref{prop:Restatement-admissibility} does not depend on $t$.
\end{definition}
%
%\begin{remark}
%\label{rem:Admissibility_and_infinite-time_admissibility}
%If the semigroup $T$ is exponentially stable, i.e. if \eqref{eq:Linear_System} is 0-UGAS, then
%$B$ is infinite-time $q$-admissible if and only if $B$ is $q$-admissible, see \cite[Lemma 2.9]{JNP18}
%or \cite[Lemma 1.1]{Gra95} (in a dual form).
%\end{remark}

\begin{lemma}
\label{lem:GrabowskiLemma}
Let $T$ be an exponentially stable semigroup and let $q \in [1,\infty]$. Then $B$ is $q$-admissible control operator iff it is infinite-time $q$-admissible control operator.
\end{lemma}

\begin{proof}
Let $q < \infty$ (the argument is analogous for $q = \infty$). 
We mimic a proof from \cite[Lemma 1.1]{Gra95}.

Clearly, infinite-time $q$-admissibility implies $q$-admissibility.
Assume that $B$ is infinite-time $q$-admissible and pick arbitrary $\tau>0$ and $u\in\Uc$.
Consider any $t=k\tau+t'$ for some $k \in \N$ and $t'<\tau$.
{\allowdisplaybreaks
\begin{align*}
 \Big\| \int_0^t & T(s)Bu(s)\,ds\Big\|_X \\
&= \left\| \int_{k\tau}^{k\tau+t'} T(s)Bu(s)\,ds +  \sum_{i=0}^{k-1} \int_{i \tau}^{(i+1) \tau} T(s)Bu(s)\,ds\right\|_X \\
&\leq  \left\| \int_{0}^{t'} T(s+k\tau)Bu(s+k\tau)\,ds \right\|_X +  \left\| \sum_{i=0}^{k-1} \int_{0}^{\tau} T(s+i\tau)Bu(s+i\tau)\,ds\right\|_X \\
&\leq   \|T(k\tau)\| \left\| \int_{0}^{t'} T(s)Bu(s+k\tau)\,ds \right\|_X +  \sum_{i=0}^{k-1} \|T(i\tau)\| \left\|\int_{0}^{\tau} T(s)Bu(s+i\tau)\,ds\right\|_X.
\end{align*}
Using Proposition~\ref{prop:Restatement-admissibility} and assuming without loss of generality that $t\mapsto h_t$ is nondecreasing, we have:
\begin{align*}
 \Big\| \int_0^t & T(s)Bu(s)\,ds\Big\|_X \\
&\leq   Me^{-\lambda k\tau} h_{t'} \Big( \int_0^{t'} \|u(s + k\tau)\|^q_U ds \Big)^{1/q}  +  \sum_{i=0}^{k-1} Me^{-\lambda i\tau} 
h_{\tau} \Big(\int_0^{\tau} \|u(s + i\tau)\|^q_U ds \Big)^{1/q} \\
&\leq   Me^{-\lambda k\tau} h_{\tau} \Big(\int_0^{t} \|u(s)\|^q_U ds \Big)^{1/q} +  \sum_{i=0}^{k-1} Me^{-\lambda i\tau} h_{\tau} \Big(\int_0^{t} \|u(s)\|^q_U ds \Big)^{1/q} \\
&\leq   \sum_{i=0}^{k} Me^{-\lambda i\tau} h_{\tau} \Big(\int_0^{t} \|u(s)\|^q_U ds\Big)^{1/q} \\
&\leq   \sum_{i=0}^{\infty} Me^{-\lambda i\tau} h_{\tau} \Big(\int_0^{t} \|u(s)\|^q_U ds\Big)^{1/q}.
\end{align*}
}
Taking $h:=M h_{\tau} \sum_{i=0}^{\infty} e^{-\lambda i\tau}$, we get the result.
\end{proof}

\mir{Was norm-to-integral ISS defined?}

Now we can characterize ISS of \eqref{eq:Linear_System}:
\begin{theorem}[ISS characterizations for linear systems with unbounded input operators]
\label{thm:ISS-Criterion-lin-sys-with-unbounded-operators}
Let $X$ and $U$ be Banach spaces and $q \in[1,\infty]$. Consider the system \eqref{eq:Linear_System} with $\phi$ defined by \eqref{eq:Lifted_Lin_Sys_mild_Solution}.
The following assertions are equivalent.

\begin{enumerate}[label=(\roman*)]
    \item\label{itm:i-ISS-Crit-Lin-Unbounded} \eqref{eq:Linear_System} is $L^q$-eISS with a linear gain.
    \item\label{itm:ii-ISS-Crit-Lin-Unbounded} \eqref{eq:Linear_System} is $L^q$-ISS.
    \item\label{itm:iii-ISS-Crit-Lin-Unbounded} $T$ is exponentially stable $\ \wedge\ $ $B$ is $q$-admissible 
		$\ \wedge \ $ (in case if $q=\infty$) $\phi$ is continuous w.r.t.\  time in the norm of $X$.
    \item\label{itm:iv-ISS-Crit-Lin-Unbounded} $T$ is exponentially stable  $\ \wedge\ $ $B$ is infinite-time $q$-admissible 
    $\ \wedge \ $ (in case if $q=\infty$) $\phi$ is continuous w.r.t.\  time in the norm of $X$.
		\item\label{itm:v-ISS-Crit-Lin-Unbounded} \eqref{eq:Linear_System} is well-posed and norm-to-integral ISS w.r.t.\  $L^q(\R_+,U)$.
\end{enumerate}
\end{theorem}

\begin{proof}
\ref{itm:i-ISS-Crit-Lin-Unbounded} $\Rightarrow$ \ref{itm:ii-ISS-Crit-Lin-Unbounded} $\Rightarrow$ \ref{itm:iii-ISS-Crit-Lin-Unbounded}. Evident.

\ref{itm:iii-ISS-Crit-Lin-Unbounded} $\Rightarrow$ \ref{itm:iv-ISS-Crit-Lin-Unbounded}. Follows by Lemma~\ref{lem:GrabowskiLemma}.

\ref{itm:iv-ISS-Crit-Lin-Unbounded} $\Rightarrow$ \ref{itm:i-ISS-Crit-Lin-Unbounded}. 
Follows from Proposition~\ref{prop:Restatement-admissibility} with $h\equiv const$ and exponential stability of a semigroup $T$.

\ref{itm:iv-ISS-Crit-Lin-Unbounded} $\Iff$ \ref{itm:v-ISS-Crit-Lin-Unbounded}. 
As \eqref{eq:Linear_System} is well-posed, the operator $B$ is $q$-admissible, and, by Propositions~\ref{prop:q-admissibility-implies-continuity}, \ref{prop:infty-admissibility-implies-continuity}, the system \eqref{eq:Linear_System} has the BRS and CEP properties. Now Theorem~\ref{thm:ncISS_LF_sufficient_condition_NEW} shows the claim.
\end{proof}

Similarly in spirit to Theorem~\ref{thm:ISS-criterion-linear-systems-bounded-operators},
Theorem~\ref{thm:ISS-Criterion-lin-sys-with-unbounded-operators} reduces the ISS analysis of linear systems to the     stability analysis of the semigroup and to admissibility analysis of the input operator, which are classical functional-analytic problems with
many powerful tools for its solution, see \cite{JaP04, TuW09}.



%\section{Linear boundary control systems}
%\label{sec:Boundary_control_systems}
%
%For many natural and engineering systems, the interaction of a system with its environment (by controls, inputs, and outputs) occurs at the boundary of the system. Examples for such behavior are given by diffusion equations \cite{AWP12}, vibration of structures \cite{CuZ95}, transport phenomena, etc., with broad applications in robotics \cite{EMJ17}, aerospace engineering \cite{BCC16, PGC13}, and additive
%manufacturing \cite{DiK15,HMR15}. Wide classes of port-Hamiltonian systems can be formulated as boundary control systems as well, see \cite{JaZ12,ScJ14}.
%
%The development of the theory of general boundary control systems has been initiated in the pioneering work \cite{Fat68}, and was brought further forward by \cite{Sal87}. In the literature, there are several ways how to define a boundary control system, see, e.g., \cite{Fat68}, \cite{CuZ95, JaZ12}, 
%\cite{Sal87,TuW09} and \cite{EmT00}. The differences between various methods are discussed in \cite{LGE00}.
%We follow here the strategy due to \cite{JaZ12}, with some motivation from \cite{EmT00}.
%
%%
%%\subsection{Boundary control systems as systems with admissible operators}
%%\label{sec:BCS-as-linear-systems}
%
%Let $X$ and $U$ be Banach spaces. Consider the system
%\begin{subequations}
%\label{eq:BCS}
%\begin{align}
%\dot{x}(t) &= {\Ah} x(t), \qquad x(0) = x_0, \label{eq:BCS-1}\\
%{\Gh}x(t) &= u(t),    \label{eq:BCS-2}
%\end{align}
%\end{subequations}
%\index{operator!formal system}
%where the \emph{formal system operator} $\Ah: D( \Ah ) \subset X \to X$ is a linear operator, the control function $u$ takes values in $U$, and the \emph{boundary operator} $\Gh : D( \Gh ) \subset X \to U$ is linear and satisfies $D(\Ah) \subset D(\Gh)$.
%\index{operator!boundary}
%
%Equations \eqref{eq:BCS} look different from the classic linear infinite-dimensional systems, studied previously: 
%\begin{equation}
%\dot{x}(t) = Ax(t) + Bu(t),
%\quad
%x(0) = x_0,
%\label{eq:BCS-standard-linear-systems}
%\end{equation}
%where $A$ is the generator of a strongly continuous semigroup, and $B$ is either a bounded or an admissible input operator.
%
%To use for the system \eqref{eq:BCS} the theory which we developed for linear systems \eqref{eq:BCS-standard-linear-systems}, we would like to transform \eqref{eq:BCS} into the form \eqref{eq:BCS-standard-linear-systems}. This can be done only under some additional assumptions.
%\begin{definition}
%\label{def:BCS}
%The system \eqref{eq:BCS} is called a~\emph{boundary control system (BCS)} if the following conditions hold:
%\begin{enumerate}
%\item[(i)] The operator $A : D(A) \to X$ with $D(A) = D({\Ah} ) \cap \ker({\Gh})$ and
    %\begin{equation}
    %Ax = {\Ah}x \qquad \text{for} \quad x\in D(A)
        %\label{eq:BSC-ass1}
    %\end{equation}
    %is the infinitesimal generator of a $C_0$-semigroup $(T(t))_{t\geq0}$ on $X$.
		%
%\item[(ii)] There is an operator $G \in \mathcal{L}(U,X)$ such that for all $u \in U$ we have $Gu \in D({\Ah})$,
    %${\Ah}G \in \mathcal{L}(U,X)$ and         
        %\begin{equation}
    %{\Gh}Gu = u, \qquad u\in U.
        %\label{eq:BSC-ass2}
    %\end{equation}
%\end{enumerate}
%The operator $G$ in this definition is sometimes called a \emph{lifting operator} (note that $G$ is not uniquely defined by the properties in the item (ii)).
%\index{operator!lifting}
%\end{definition}
%
%Item (i) of Definition~\ref{def:BCS} shows that for $u\equiv 0$ the equations \eqref{eq:BCS} are well-posed.
%In particular, as $A$ is the generator of a certain strongly continuous semigroup $T(\cdot)$, for any $x\in D(A)$ it holds that $T(t)x \in D(A)$ and thus $T(t)x \in \ker({\Gh})$ for all $t\geq 0$, which means that \eqref{eq:BCS-2} is satisfied.
%
%Item (ii) of Definition~\ref{def:BCS} implies in particular that the range of the operator ${\Gh}$ equals $U$, and thus the values of inputs are not restricted.
%
%\begin{definition}
%\label{def:Classical-solution-for-Boundary-Control-System} 
%Consider the BCS \eqref{eq:BCS}.
%A function $x : [0, \tau] \to X$ is called a~\emph{classical solution of \eqref{eq:BCS} on $[0,\tau]$} if $x$ is continuously differentiable, $x(t) \in D({\Ah})$ for
%all $t \in [0, \tau]$, and $x(t)$ satisfies \eqref{eq:BCS} for all $t \in [0, \tau]$.
%
%The function $x : [0,\infty) \to X$ is called a~\emph{classical solution of \eqref{eq:BCS} on $[0,\infty)$} if $x$ is a~classical solution on $[0, \tau]$ for every $\tau > 0$.
%\end{definition}
%
%The next theorem gives a representation for the (unique) solution of \eqref{eq:BCS} \emph{for smooth enough inputs}.
%\begin{theorem}
%\label{thm:BCS-classical-solution-Representation}
%Consider the BCS \eqref{eq:BCS}.
%For all $u \in C^2([0,\tau],U)$, all $x_0\in X$: $x_0 - Gu(0) \in D(A)$ and all $\tau\geq 0$ the classical solution $\phi(\cdot,x_0,u)$ of \eqref{eq:BCS} on $[0,\tau]$ exists, is unique and can be represented as
%\begin{subequations}
%\label{eq:BCS-solution-for-smooth-inputs}
%\begin{align}
%\phi(t,x_0,u) &= T(t)\big(x_0-Gu(0)\big)  + \int_0^t T(t-r)\big({\Ah}Gu(r)-G\dot{u}(r)\big) dr + Gu(t) \label{eq:BCS-solution-for-smooth-inputs-1}\\
%&= T(t)x_0 + \int_0^t T(t-r){\Ah}Gu(r)dr - A\int_0^t T(t-r)Gu(r) dr \label{eq:BCS-solution-for-smooth-inputs-2}\\
%&= T(t)x_0 + \int_0^t T_{-1}(t-r)({\Ah}G - A_{-1}G)u(r)dr \label{eq:BCS-solution-for-smooth-inputs-3},
%\end{align}
%\end{subequations}
%where $A_{-1}$ and $T_{-1}$ are the extensions of the infinitesimal generator $A$ and of the semigroup $T$ to the extrapolation space $X_{-1}$, respectively.
%Furthermore, $A_{-1}G \in L(U,X_{-1})$ (and thus ${\Ah}G - A_{-1}G \in L(U,X_{-1})$).
%\end{theorem}
%
%\begin{proof}
%For \eqref{eq:BCS-solution-for-smooth-inputs-1} see \cite[Theorem 11.1.2]{JaZ12}.
%For \eqref{eq:BCS-solution-for-smooth-inputs-2} see \cite[Lemma 13.1.5]{JaZ12}.
%These results are stated in \cite{JaZ12} for Hilbert spaces, but the argumentation is valid for Banach spaces as well.
%
%The representation formula \eqref{eq:BCS-solution-for-smooth-inputs-3} seems to be well-known for the specialists in the semigroup theory. In our argument, we follow \cite[Theorem 4.4]{MiP20}.
%
%Let $A_{-1}$ be the extension of $A$ to the extrapolation space $X_{-1}$, and let $T_{-1}$ be the extrapolated semigroup, generated by $A_{-1}$.
%Note that $G\in L(U,X)$, and $D(A_{-1})=X$. Thus, the operator $A_{-1}G$ is well-defined as a linear operator from the Banach space $U$ to the Banach space $X_{-1}$ with $D(A_{-1}G) = U$. As $A_{-1}$ is the generator of a strongly continuous semigroup, it is closed.
%\ifnothabil	\sidenote{\mir{Thus, by Proposition~\ref{prop:Closed_plus_bounded_is_closed}}}\fi
%Thus, by \cite[Proposition A.9]{HMM13} the operator $A_{-1}G$ is closed as a product of a closed and a bounded operator. By closed graph theorem  $A_{-1}G \in L(U,X_{-1})$.
%\ifnothabil	\sidenote{\mir{By closed graph theorem (Theorem~\ref{thm:ClosedGraphTheorem})}}\fi
%
%\ifnothabil	\sidenote{\mir{(even for any $u \in L^{1}_{\loc}([0,\tau],U)$, see Theorem~\ref{Milde_Loesungen})}}\fi
%The map $r \mapsto T(t-r)Gu(r)$ is Bochner integrable in the space $X$ and thus also in $X_{-1}$ (even for any $u \in L^{1}_{\loc}([0,\tau],U)$, see \cite[Lemma 10.1.6]{JaZ12}).
%%\cite[Proposition 1.3.4]{ABH11}).
%Furthermore, $T(t-r)Gu(r) \in X = D(A_{-1})$.
%
%As a semigroup commutes with its infinitesimal generator, $A_{-1}T_{-1}(s)=T_{-1}(s)A_{-1}$ for all $s\in\R_+$ on $D(A_{-1})$. 
%Consider the map 
%\[
%w:r \mapsto A_{-1}T_{-1}(t-r)Gu(r) = T_{-1}(t-r)A_{-1}Gu(r).
%\]
%\ifnothabil	\sidenote{\mir{the function $w$ is Bochner integrable on $X_{-1}$, by Theorem~\ref{Milde_Loesungen}.}}\fi
%Since $A_{-1}G \in L(U,X_{-1})$ and $T_{-1}$ is a strongly continuous semigroup on $X_{-1}$, the function $w$ is 
%Bochner integrable on $X_{-1}$, by \cite[Lemma 10.1.6]{JaZ12}.
%\ifnothabil	\sidenote{\mir{Hence, Lemma~\ref{lem:Commutation_Closed_integral} can be applied }}\fi
%Hence, \cite[Proposition 1.3.4]{ABH11} can be applied to obtain for all $u \in C^2([0,\tau],U)$ that
%\begin{align*}
%A\int_0^t T(t-r)Gu(r) dr &= A_{-1}\int_0^t T_{-1}(t-r)Gu(r) dr \\
%&= \int_0^t A_{-1} T_{-1}(t-r)Gu(r) dr = \int_0^t  T_{-1}(t-r)A_{-1}Gu(r) dr.
%\end{align*}
%From this the formula \eqref{eq:BCS-solution-for-smooth-inputs-3} follows.
%\end{proof}
%
%An advantage of the representation formula \eqref{eq:BCS-solution-for-smooth-inputs-1} is in the boundedness of the operators $G$ and $\Ah G$, involved in the expression, but the disadvantage is that the derivative of $u$ is employed.
%Still, the expression on the right-hand side of \eqref{eq:BCS-solution-for-smooth-inputs-1} makes sense for any $x \in X$ 
%and for any $u \in H^1([0,\tau],U)$, and can be called a mild solution of the BCS \eqref{eq:BCS}, as is done, e.g., in \cite[p. 146]{JaZ12}.
%
%The formula \eqref{eq:BCS-solution-for-smooth-inputs-3} does not involve any derivatives of inputs, and again is given in terms of the bounded operator ${\Ah}G - A_{-1}G \in L(U,X_{-1})$.
%Moreover, if we consider the expression in the right-hand side of \eqref{eq:BCS-solution-for-smooth-inputs-3} in the extrapolation spaces $X_{-1}$, then it makes sense for all $x \in X$ and all $u\in L^{1}_{\loc}(\R_+,U)$, and defines a mild solution (in the space $X_{-1}$) of the equation 
%\begin{eqnarray}
%\dot{x} = A_{-1}x + ({\Ah}G-A_{-1}G)u.
%\label{eq:BCS:State-space-representation}
%\end{eqnarray}
%
%\begin{remark}
%\label{rem:BCS-are-linear-abstract-systems} 
%As we have shown, any BCS \eqref{eq:BCS} on a Banach space $X$ can be reformulated as a linear system with a bounded input operator in $X_{-1}$. 
%For the converse statement, see \cite[Remark 2.10]{Sch20}.
%%\mir{Possibly: add a reference where the converse statement has been shown.}
%\end{remark}
%
%As we know from Theorem~\ref{thm:BCS-classical-solution-Representation}, 
%for all $u \in C^2([0,\tau],U)$, all $x_0\in X$: $x_0 - Gu(0) \in D(A)$ and for all $\tau\geq 0$
%the value of the expression on the right-hand side of \eqref{eq:BCS-solution-for-smooth-inputs-3} lies in $X$.
%
%However, to ensure that the integral term in \eqref{eq:BCS-solution-for-smooth-inputs-3} belongs to $X$ for less regular $u$, we have to require that the input operator 
%\begin{eqnarray}
%B:={\Ah}G-A_{-1}G
%\label{eq:BCS-Input-Operator}
%\end{eqnarray}
%has some sort of admissibility. 
%
%\begin{remark}
%\label{rem:Uniqueness-of-B-boundary-control-systems} 
%The operator $B$ is uniquely defined by the boundary control system, and does not depend on the choice of the lifting operator $G$, see \cite[Proposition 2.8]{Sch20}.
%\end{remark}
%
%\begin{definition}
%\label{def:Mild-solution-for-Boundary-Control-System} 
%Let $q\in[1,\infty]$ be given. If the input operator $B$ defined by \eqref{eq:BCS-Input-Operator} is $q$-admissible for $A$, then for each $x_0\in X$ and each $u\in L^q(\R_+,U)$
%the function $\phi(\cdot,x_0,u):\R_+\to X$, defined by \eqref{eq:BCS-solution-for-smooth-inputs-3}, is called the \emph{mild solution of the BCS \eqref{eq:BCS}}.
%\end{definition}
%
%%
%%\subsection{Input-to-state stability of boundary control systems}
%%\label{sec:ISS-of-BSC}
%%
%%Having the representations \eqref{eq:BCS-solution-for-smooth-inputs} (for smooth inputs) and \eqref{eq:BCS:State-space-representation} (for general inputs) for solutions of BCS \eqref{eq:BCS},
%%we can apply the criteria for ISS of  general linear systems for ISS analysis of BCS.
%
%%\startCP
%%In the next corollary and its proof, $p$ could be $p=\infty$. Correct?
%%\stopCP
%
%\begin{corollary}
%\label{cor:ISS-for-BCS} 
%Consider the boundary control system \eqref{eq:BCS} and assume that the corresponding input operator $B$ defined by 
%\eqref{eq:BCS-Input-Operator} is $q$-admissible for some $q\in [1,+\infty)$. Assume that $A$ generates an exponentially stable semigroup.
%Then for any $p\in[q,+\infty]$
%the system $\Sigma:=(X,\Uc,\phi)$ with $\Uc:=L^p(\R_+,U)$ is an ISS control system (with respect to the norm in $\Uc$).
%\end{corollary}
%
%\begin{proof}
%As $B$ defined by \eqref{eq:BCS-Input-Operator} is $q$-admissible for some $q\in [1,+\infty)$, then it is $p$-admissible for any $p\in[q,+\infty]$ and furthermore, the map $\phi$ is continuous w.r.t.\ time. 
%By Proposition~\ref{prop:q-admissibility-implies-continuity}, for all $p\in[q,+\infty]$, the system $\Sigma:=(X,\Uc,\phi)$ with $\Uc:=L^p([0,\infty),U)$, is a forward-complete control system in the sense of Definition~\ref{Steurungssystem}. 
%By Theorem~\ref{thm:ISS-Criterion-lin-sys-with-unbounded-operators}, the system $\Sigma$ is ISS.
%\end{proof}
%
%\begin{remark}
%\label{rem:Weak solutions of boundary control systems}
%In this chapter, we consider mild solutions of boundary control systems. 
%In some papers, the concepts of weak solutions and strong solutions are used. 
%For a detailed discussion of the relationship between all these solution concepts we refer to \cite[Propositions 2.9, 2.11, Remark 2.10]{Sch20}. 
%\end{remark}
%
%%\begin{remark}
%%\label{rem:Further-results} 
%%Certain further functional-analytic insights on linear boundary\linebreak control systems one can find in \cite{Sch20}.
%%\end{remark}
%
%%
%%Now we proceed to study of stability properties of boundary control systems.
%%First of all, using Theorem~\ref{thm:Fattorini-trick}, we can prove that all 0-UGAS boundary control systems are ISS with respect to the inputs and their derivatives.
%%
%%
%%\mir{One should choose nice input spaces so that the derivative of the input exists and is again in a nice space.}
%%
%%
%%\begin{definition}
%%\label{def:D1-ISS} 
%%Let $\Sigma:=(X,\Uc,\phi)$ be a control system, and let $\Uc:=H^1([0,\tau],U)$ for a certain normed vector space $U$.
%%We call $\Sigma$ $D^1$-ISS, if there are $\beta\in\KL$ and $\gamma_0,\gamma_1\in\Kinf$ so that 
%%for all $x\in X$, all $u\in\Uc$ and $t\geq 0$ it holds that
%%\begin{eqnarray}
%%\|\phi(t,x,u\|_X\leq \beta(\|x\|_X,t) + \gamma_0(\|u\|_\Uc) + \gamma_1(\|\dot{u}\|_\Uc).
%%\label{eq:D1-ISS}
%%\end{eqnarray}
%%\end{definition}
%
%
%
%%\subsection{Example}
%%\label{sec:Example}
%%
%%As an example, consider the following linear heat equation.
%%\begin{eqnarray}
%%x_t(t,z) = \mu x_{zz}(t,z)
%%\label{eq:Linear_Diffusion-Dirichlet-control}
%%\end{eqnarray}
%%with a Dirichlet boundary input $u$:
%%\begin{eqnarray}
%%x(t,0)&=& 0 ,\quad t>0\\
%%x(t,1)&=& u(t), \quad t>0.
%%\label{eq:DirichletConditions_Linear_Diffusion-Dirichlet}
%%\end{eqnarray}
%%We assume that $X:=L^2(0,1)$ and $\Uc:=PC(\R_+,\R)$.
%%
%%\mir{I am not sure that $\Uc:=PC(\R_+,\R)$ is a good choice. I have to go for more general input spaces.}
%%
%%Interpreting $x(t,z)$ as the temperature of a body in a position $z\in[0,1]$ at time $t\geq 0$, the sense of the boundary condition \eqref{eq:DirichletConditions_Linear_Diffusion} is that at the end $z=0$ the zero temperature is maintained, and at the end $z=1$ we can regulate the temperature by means of a control $u$.
%%
%%This system can be naturally written in the form \eqref{eq:BCS}
%%where:
%%\begin{itemize}
    %%\item the formal system operator $\Ah$ is given by
    %%\begin{eqnarray}
    %%\Ah x= \frac{d^2 x}{dx^2},\quad x \in D(\Ah) := H^2(0,1) \cap H^1_L(0,1),
    %%\label{eq:Formal-system-operator-Heat}
    %%\end{eqnarray}
    %%with 
    %%\begin{eqnarray}
    %%H^1_L(0,1) := \{g\in H^1(0,1): g(0)=0\}.
    %%\label{eq:H1L-definition}
    %%\end{eqnarray}
%%
    %%\item The \emph{boundary operator} $\Gh:X \to \R$ is given by 
    %%\begin{eqnarray}
    %%\Gh (x) = x(1),\quad x \in D(\Gh) := H^2(0,1) \cap H^1_L(0,1),
    %%\label{eq:Boundary-opertator-Heat}
%%\end{eqnarray}
%%
    %%\item $u(t) \in \R$
%%\end{itemize}
%%
%%Before we analyze the general case let us see how this works in the case of systems \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}, 
%%\eqref{eq:Linear_Diffusion-Dirichlet-control}.
%%
%%Assume that $u$ is a continuously differentiable input and that $x$ is a corresponding classical solution of a system 
%%\eqref{eq:Linear_Diffusion-Dirichlet-control}, \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}.
%%Define
%%\begin{equation*}
%%v(z, t) = x(z, t) - z u(t),\quad z\in[0,1],\ t\geq 0.
%%\end{equation*}
%%We obtain the following partial differential equation for $v$:
%%\begin{eqnarray*}
%%v_t(z, t) & =& v_{zz} (z, t) - z\dot{u}(t), \qquad z\in[0, 1], \quad t \geq0\\
%%v(0,t) &=& v(1, t) = 0,\quad t\geq0.
%%\end{eqnarray*}
%%This partial differential equation for $v$ is a system with a distributed control $\tilde{u} := \dot{u}$, which can be represented as an abstract evolution equation
%%\begin{equation*}
%%\dot{v}(t) = Av(t) + \tilde{B}\tilde{u}(t)
%%\end{equation*}
%%for a certain infinitesimal generator $A$ and a bounded operator $\tilde{B}$.
%%Thus, for smooth inputs a system 
%%\eqref{eq:Linear_Diffusion-Dirichlet-control}, \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}
%%with boundary inputs can be converted into the classical form \eqref{eq:BCS-standard-linear-systems}.
%%At the same time, one can show that the system \eqref{eq:Linear_Diffusion-Dirichlet-control},
%%\eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet} \emph{cannot} be written in a form \eqref{eq:BCS-standard-linear-systems} \emph{for all inputs in $\Uc$ with a bounded operator $B$}, see Exercise~\ref{ex:BCS-Transport-equation}, item (iii) for the same question for the transport equation.
%




==> chap_Linear_Systems.tex <==


\chapter{Linear systems with unbounded input operators}
\label{chap:ISS_linear_systems}


\todo{
Plan:

\begin{itemize}
	\item Section~\ref{sec:Linear_systems} is an expanded version (with some proofs) of the section which I have written for the SIREV paper with Christophe.
	This should be a core for the chapter.
	\item Section~\ref{sec:Wei89b-to-rewrite} is a copy-paste of some results and proofs from Wei89b. Must be completely rewritten and embedded into other material.
	\item Section~\ref{sec:Boundary control systems} is a copy-paste of some results and proofs from JaZ12. Must be completely rewritten and embedded into other material.
	\item The rest contains some of the proofs, which can be embedded into the stuff in Section~\ref{sec:Linear_systems}.
\end{itemize}
}



{\color{red}\LARGE
\textbf{
\begin{center}
Some older stuff follows
\end{center}
}
}


What gives us a linear theory:

\begin{itemize}
	\item A basic understanding of the infinite-dimensional theory
	\item A basis for the proof of existence and uniqueness results for the nonlinear systems (together with various fixed-point theorems)
	\item Knowledge of the spectral properties of the generators of the semigroups
	\item Inequalities in Sobolev spaces (as Friedrich's inequality). They are then crucial for the Lyapunov theory of nonlinear systems with distributed as well as boundary inputs.
\end{itemize}


\ifAndo
{\color{red}
\section{Some stuff from Wei89b}
\label{sec:Wei89b-to-rewrite}

\todo{Must be rewritten, changed and adapted for the rest of the text. Now it is just copypaste.}


\begin{proposition}\label{prop:Proposition_2.3}
Let $X$ and $\Omega$ be as in Definition {2.1} with $p < \infty$ and
let $\Sigma=(\mathbb{T},\Phi)$ be an abstract linear control system
on $X$ and $\Omega$. Then the function
\begin{gather*}
q(t, u) = \Phi_t u
\end{gather*}
is continuous on the product $[0, \infty) \times \Omega$, in
particular $\Phi=(\Phi_t)_{t\geq0}$ is a~strongly continuous family of operators.
\end{proposition}

\begin{proof}
Taking in {(2.1)} $u=0$ and taking the supremum for $\|v\|=1$ we get,
denoting $T=\tau+t$,
\begin{equation}
\|\Phi_t\| \leqq \|\Phi_{T}\|
\quad\text{for}\quad
t\leqq T,
\label{eq:Book_2.3}
\end{equation}
i.e., $\|\Phi_t\|$ is nondecreasing.

Let us first prove the continuity of $\varphi(t, u)$ with
respect to the time $t$, so for the time being let $u\in\Omega$ be fixed and
let
\begin{gather}
f(t)=\Phi_t u.
\end{gather}
Inequality \eqref{eq:Book_2.3} together with causality {(2.2)} implies that
for $t\in[0, 1]$
\begin{gather}
\|f(t)\| \leqq \|\Phi_1\|\cdot\|P_t u\|.
\end{gather}
Obviously $\|\Phi_t u\| \to 0$ for $t \to 0$
(because of $p<\infty$), so
\begin{gather}
\lim_{t\to0}f(t) = 0.
\end{gather}
The right continuity of $f$ in any $\tau > 0$ now follows easily from the
composition property {(2.1)}.
To prove the left continuity of $f$ in $\tau>0$
we take a~sequence $(\varepsilon_n)$ with
$\varepsilon_n \in [0, \tau]$ and $\varepsilon_n \to 0$ and define
$u_n(t)=u(\varepsilon_n+t)$, so $u_n \to u$ (because of $p<\infty$).
We have
\begin{gather*}
u = u \Diam{\varepsilon_n} u_n,
\end{gather*}
so according to {(2.1)}
\begin{gather*}
\Phi_{\varepsilon_n+(\tau-\varepsilon_n)}u
 = \mathbb{T}_{\tau-\varepsilon_n}\Phi_{\varepsilon_n}u
 + \Phi_{\tau-\varepsilon_n} u_n.
\end{gather*}
From here
\begin{gather*}
\Phi_{\tau}u - \Phi_{\tau-\varepsilon_n}u
 = \mathbb{T}_{\tau-\varepsilon_n}\Phi_{\varepsilon_n}u
 + \Phi_{\tau-\varepsilon_n}(u_n-u),
\end{gather*}
which yields
\begin{gather*}
\|\Phi_{\tau}u - \Phi_{\tau-\varepsilon_n}u\|
 \leqq M \cdot \|f(\varepsilon_n)\| + \|\Phi_{\tau}\| \cdot \|u_n-u\|,
\end{gather*}
where $M$ is a~bound for $\|\mathbb{T}_t\|$ on $[0,\tau]$.
Thus the left continuity of $f$
in any $\tau > 0$ is also proved.

The joint continuity of $\varphi$ follows
easily now from the decomposition
\begin{gather}
\Phi_t v - \Phi_{\tau}u = \Phi_t(v-u) + (\Phi_t-\Phi_{\tau})u
\end{gather}
where $(t, v)\to(\tau, u)$.
\end{proof}

\begin{problem}\label{Problem_2.4}
In the above proof we have twice used the fact
that $p<\infty$. I do not know if the proposition holds for $p=\infty$.
\end{problem}

We give an estimate for the growth rate of $\|\Phi_t\|$.

\begin{proposition}\label{prop:Proposition_2.5}
Let $X$ and $\Omega$ be as in Definition {2.1}
and let $(\mathbb{T},\Phi)$ be an abstract linear control system
on $X$ and $\Omega$.

If $M \geqq 1$ and $\omega > 0$ are such that
\begin{gather}
\|\mathbb{T}_t\| \leqq M e^{\omega t}
\qquad
\forall t\geqq0,
\end{gather}
then there is some $L\geqq0$ such that
\begin{gather*}
\|\Phi_t\| \leqq L e^{\omega t}
\qquad
\forall t\geqq0.
\end{gather*}
\end{proposition}


\begin{proof}
From {(2.1)} we get through induction
\begin{equation}
\Phi_n\left( \dots \left(u_1\Diam{1}u_2\right)\Diam{2}
 \dots \Diam{n-1}u_n\right)
 = \mathbb{T}_{n-1} \Phi_1 u_1
 + \mathbb{T}_{n-2} \Phi_1 u_2
 + \dots
 + \Phi_1 u_n,
\label{eq:Book_2.4}
\end{equation}
whence for $t \in (n-1, n]$ (using \eqref{eq:Book_2.3})
\begin{gather*}
\|\Phi_t\| \leqq \|\Phi_n\|
 \leqq \big(\|\mathbb{T}_{n-1}\|+\|\mathbb{T}_{n-2}\|+\dots+\|I\|)
 \cdot \|\Phi_1\|
 \leqq M \frac{e^{\omega n}-1}{e^{\omega}-1}\|\Phi_1\|,
\end{gather*}
so we can take
\begin{gather*}
L = M \frac{e^{\omega}}{e^{\omega}-1}\|\Phi_1\|.
\end{gather*}
\end{proof}

\begin{remark}\label{rem:Remark_2.6}
For $\omega=0$, $\Phi$ does not have to be uniformly bounded but we
can easily obtain from \eqref{eq:Book_2.4},
using the Cauchy--H\"{o}lder inequality,
that
\begin{gather*}
\|\Phi_t\| \leqq L \cdot (1+t)^{1-1/p}
\quad
\forall t\geqq0,
\end{gather*}
for some $L \geqq 0$. For $\omega < 0$, $\Phi$ is uniformly bounded.
\end{remark}

\begin{definition}\label{Definition_3.1}
Let $X$ be a~Banach space and $\mathbb{T}$ a~strongly
continuous semigroup on $X$ with generator $A : D(A) \to X$.
Let $\beta\in\rho(A)$,
the resolvent set of $A$ (if $X$ is real, take $\beta\in\mathbb{R}$).
We define the space
$X_1$ to be $D(A)$ with the norm
\begin{gather*}
\|x\|_1 = \|(\beta I - A)x\|,
\end{gather*}
and the space $X_{-1}$ to be the completion
of $X$ with respect to the norm
\begin{gather*}
\|x\|_{-1} = \|(\beta I - A)^{-1}x\|.
\end{gather*}
\end{definition}

\begin{definition}\label{Definition_3.5}
Let $X$ be a~Banach space, let $\mathbb{T}$ be a~semigroup on $X$
with generator $A$, and let
\begin{gather*}
f \in L^1_{loc}([0,\infty), X_{-1}).
\end{gather*}
Then we say that the function
\begin{gather*}
x(\cdot) \in L^1_{loc}([0,\infty), X)
\end{gather*}
is a~\emph{strong solution} of the
differential equation
\begin{equation}
\dot{x}(t) \in Ax(t)+f(t)
\label{eq:Book_3.1}
\end{equation}
if for any $t \geq O$
\begin{gather*}
x(t)-x(0) = \int_0^t \left[Ax(s)+f(s)\right] ds.
\end{gather*}
If additionally, $x(\cdot)$ is continuous in $X$,
i.e., if
\begin{gather*}
x(\cdot) \in C([0,\infty),X),
\end{gather*}
then we say that $x(\cdot)$ is a~\emph{continuous
state strong solution} of the differential equation above.
\end{definition}

\begin{theorem}
\label{thm:Representation-abstract-systems}
Let $U$ and $X$ be Banach spaces, let $p \in [1,\infty)$, and let
$\Omega = L^p([0,\infty), U)$.
Let $(\mathbb{T},\Phi)$ be an abstract linear control system
on $X$ and $\Omega$.
Then there is a~unique operator $B \in \mathcal{L}(U, X_{-1})$ such that for
any $u\in\Omega$ and any $t\geq0$
\begin{equation}
\Phi_t u = \int_0^t \mathbb{T}_{t-\sigma} Bu(\sigma)d\sigma.
\label{eq:Book_3.2}
\end{equation}
Moreover, for any $X_0 \in X$ and $u \in \Omega$
the function of $t \geq 0$
\begin{equation}
x(t) = \mathbb{T}_t x_0 + \Phi_t u
\label{eq:Book_3.3}
\end{equation}
is the (unique)
continuous state strong solution of the differential equation
\begin{equation}
\dot{x}(t)=Ax(t)+Bu(t)
\label{eq:Book_3.4}
\end{equation}
with
\begin{gather*}
x(0)=x_0.
\end{gather*}
\end{theorem}

}
\fi






\section{Boundary control systems}
\label{sec:Boundary control systems}



\subsection{Plan for the survey}

\begin{itemize}
	\item Read about Sobolev spaces
	\begin{itemize}
		\item Sobolev spaces and Bochner integrals HMM13, Appendix F.
		\item HiP00, where we could read it as well.
		\item The appendix in CuZ95 would be also an interesting thing.
		\item Write down the main ideas on Sobolev spaces.
		\item Write the Section on boundary control systems in SIREV Paper.
		\item Read well-posedness chapter in JaZ12
	\end{itemize}
	\item Read JaZ12, TuW09, CuZ95, Section 3.3
	\item Further papers: Fat68, GCM05, Sle76,
	\item ScZ18, LhS18
	\item D-ISS for 0-UGAS boundary control systems
	\item ISS analysis.

	\item Nonlinear systems
\begin{itemize}
	\item Probably realize the same technique for nonlinear systems, as Jochen did in his work with Hans.
	\item Think about: we could try another idea: first use the Dirichlet lifting (or the Fattorini's trick) to reformulate the original boundary control system in a form which involves the derivatives of the input. 
	
\end{itemize}

\end{itemize}



\subsection{Plan for a paper, work title "Input-to-state stability of boundary control systems"}


As I understand, there are 2 ways how to reformulate the boundary control system into the standard formulation:
\begin{itemize}
	\item[(i)] Using Fattorini's trick
	\item[(ii)] Other approach to construct admissible operators.
\end{itemize}
In the first case we obtain a system whose dynamics depends not only on the inputs $u$, but also on $\dot{u}$.


\subsubsection{Linear systems}


The modified system has only bounded input operators applied to inputs $u$ and $\dot{u}$, and thus we can ask whether:
\begin{itemize}
	\item Modified system is $D^1$-ISS provided the modified system is 0-UGAS. 
	\item Original BC system is $D^1$-ISS provided the original BC system is 0-UGAS. 
\end{itemize}

Admissibility approach: it would be great to relate the results of Birgit and Felix to the BCS.
\begin{itemize}
	\item Can we construct the operators $A$ and $B$ for the admissibility form explicitly?
	\item Can we formulate the conditions on ISS of the BC system directly in terms of the data on a boundary control system, and not on the data of the obtained system in the admissibility form?
\end{itemize}

\subsubsection{Nonlinear systems}

\begin{itemize}
	\item We have to obtain an equivalent modified equation for a nonlinear BC system.
	\item A result on $D^1$-ISS of the original system.
\end{itemize}

Lyapunov functions for boundary control systems
\begin{itemize}
	\item Currently we have tried to construct ISS Lyapunov functions for the systems with admissible operators. But may be it will be easier and more understandable to construct them for BC systems directly?
\end{itemize}

Monotone systems:
\begin{itemize}
	\item We have the relation on the flows of the original and modified system. Can we show then that the BC system is monotone iff the modified system is monotone?
	\item Maybe we can even start the estimations by the maximum and minimum solutions already for a modified system and not for the original BC system. 
	\item Final aim is to show that a monotone system is ISS if and only if the modified system is ISS.
				As a particular case show that for a linear monotone BC system ISS is equivalent to 0-UGAS.
	\item 
\end{itemize}


I think that it would be possible also to write a DFG grant on 'ISS for boundary control systems', based on these ideas.
Possible WPs are:
\begin{itemize}
	\item ISS of linear boundary control systems
	\item ISS of nonlinear boundary control systems
	\item ISS Lyapunov methods for BC systems.
	\item Monotone boundary control systems
	\item Applications:
	\begin{itemize}
		\item ???
	\end{itemize}
	
\end{itemize}






\subsection{Boundary  control systems}
\label{sec:BSC}


For many natural and engineering systems the interaction of the systems with its environment (by controls, inputs and outputs) occurs only at the boundary of the system. 
This kind of systems naturally appears in numerous boundary control problems such as 
diffusion or diffusive equations \cite{AWP12}, vibration of structures \cite{CuZ95}, transport phenomena, with broad applications in robotics \cite{EMJ17}, aerospace engineering \cite{PGC13}, \cite{BCC16}, and additive
manufacturing \cite{DiK15}, \cite{HMR15}. Broad classes of port-Hamiltonian systems can be formulated as boundary control systems as well, see \cite{ScJ14,JaZ12}.
Theory of general boundary control systems initiated in a seminal paper \cite{Fat68} gives a unified method to analyze such problems.
Consider a system
\begin{subequations}
\label{eq:BCS}
\begin{eqnarray}
\dot{x}(t) &=& {\Ah} x(t), \qquad x(0) = x_0, \label{eq:BCS-1}\\
{\Gh}x(t) &=& u(t),    \label{eq:BCS-2}
\end{eqnarray}
\end{subequations}
where the \emph{formal system operator} $\Ah: D( \Ah ) \subset X \to X$ is a linear operator, the control function $u$ takes values in the
Hilbert space $U$, and the \emph{boundary operator} $\Gh : D( \Gh ) \subset X \to U$ is linear and satisfies $D(\Ah) \subset D(\Gh)$.

Equations \eqref{eq:BCS} look rather differently than the classic linear infinite-dimensional systems, studied previously: 
\begin{equation}
\dot{x}(t) = Ax(t) + Bu(t),
\quad
x(0) = x_0.
\label{eq:BCS-standard-linear-systems}
\end{equation}
where $A$ is a generator of a strongly continuous semigroup, and $B$ is either bounded or admissible input operator.

In order to use for BCS \eqref{eq:BCS} the theory which we developed for linear systems \eqref{eq:BCS-standard-linear-systems}, we would like to transform the system \eqref{eq:BCS} into the form \eqref{eq:BCS-standard-linear-systems}. This can be done only under some additional assumptions.
\begin{definition}
\label{def:BCS}
The system \eqref{eq:BCS} is called a~\emph{boundary control system (BCS)} if the following conditions hold:
\begin{enumerate}
\item[(i)] The operator $A : D(A) \to X$ with $D(A) = D({\Ah} ) \cap \ker({\Gh})$ and
    \begin{equation}
    Ax = {\Ah}x \qquad \text{for} \quad x\in D(A)
		\label{eq:BSC-ass1}
    \end{equation}
    is the infinitesimal generator of a strongly continuous semigroup $(T(t))_{t\geq0}$ on $X$;
\item[(ii)] There is an operator $G \in \mathcal{L}(U,X)$ such that for all $u \in U$ we have $Gu \in D({\Ah})$,
    ${\Ah}G \in \mathcal{L}(U,X)$ and 		
		\begin{equation}
    {\Gh}Gu = u, \qquad u\in U
		\label{eq:BSC-ass2}
    \end{equation}
\end{enumerate}
The operator $G$ in this definition is sometimes called a \emph{lifting operator}.
\end{definition}
Item (i) of the definition shows that for $u\equiv 0$ the equations \eqref{eq:BCS} are well-posed.
In particular, as $A$ is the generator of a $C_0$-semigroup, for the corresponding semigroup $T$ and for any $x\in D(A)$ it holds that $T(t)x \in D(A)$ and thus $T(t)x \in \ker({\Gh})$ for all $t\geq 0$, which means that the second equation in \eqref{eq:BCS} is satisfied.

Item (ii) of the definition implies in particular that the range of the operator ${\Gh}$ equals $U$, and thus the values of an inputs are not restricted.

\begin{definition}
\label{def:Classical-solution-for-Boundary-Control-System} 
Consider a BCS \eqref{eq:BCS}.

The function $x : [0, \tau] \to X$ is called a~\emph{classical solution of \eqref{eq:BCS} on $[0,\tau]$} if $x$ is a~continuously differentiable function, $x(t) \in D({\Ah})$ for
all $t \in [0, \tau]$, and $x(t)$ satisfies \eqref{eq:BCS} for all $t \in [0, \tau]$.

The function $x : [0,\infty) \to X$ is called a~\emph{classical solution of \eqref{eq:BCS} on $[0,\infty)$} if $x$ is a~classical solution on $[0, \tau]$ for every $\tau > 0$.
\end{definition}

In the next theorem we show that \emph{for smooth enough inputs} \eqref{eq:BCS} can be reformulated as an abstract differential equation \eqref{eq:BCS-standard-linear-systems} with a bounded operator $B$.

\begin{theorem}
\label{thm:Fattorini-trick}
Consider the boundary control system \eqref{eq:BCS} and the abstract differential equation 
\begin{equation}
\dot{v}(t) = Av(t) - G\dot{u}(t) + {\Ah}Gu(t),
\qquad
v(0) = v_0.
\label{eq:Book_11.6}
\end{equation}
Assume that $u \in C^2([0,\tau];U)$. Then the classical solution of \eqref{eq:Book_11.6} exists and is unique for any $v_0\in D(A)$.
Furthermore, if $v_0 = x_0 - Gu(0) \in D(A)$, then the classical
solutions of \eqref{eq:BCS} and \eqref{eq:Book_11.6} on $[0, \tau]$
are related by
\begin{equation} 
\label{eq:Book_11.7}
v(t) = x(t) - Gu(t)
\end{equation}
and the classical solution of \eqref{eq:BCS} is unique.
\end{theorem}

\begin{proof}
Since $A$ is the infinitesimal generator of a
$C_0$-semigroup and $G$ and ${\Ah}G$ are bounded linear operators (by assumptions of Definition~\eqref{def:BCS}, that equation \eqref{eq:Book_11.6} has a~unique classical solution
for $v_0 \in D(A)$ and $u \in C^2([0,\tau];U)$.

Now let the condition $v_0 = x_0 - Gu(0) \in D(A)$ holds. 
Assume that $x$ is a~classical solution of \eqref{eq:BCS}.
Then for $t \in [0, \tau]$ we have that ${\Gh}x(t) = u(t)$ and furthermore
\begin{equation*}
{\Gh}v(t) = {\Gh}\big(x(t) - Gu(t)\big) = {\Gh}x(t) -{\Gh}Gu(t) = 0.
\end{equation*}
where we have used that \eqref{eq:BSC-ass2} holds.

%
%
%$v(t) \in D(A) \subset D({\Ah}) \subset D({\Gh})$,
%$Gu(t) \in D({\Gh})$, and
%since
%$v(t) \in D(A) \subset \ker{\Gh}$ and
%the equation \eqref{eq:BSC-ass2} holds, we obtain that
%\begin{equation*}
%{\Gh}x(t) = {\Gh}(v(t) + Gu(t))
 %= {\Gh}v(t) +{\Gh}Gu(t) = u(t).
%\end{equation*}

Furthermore, equation \eqref{eq:Book_11.7} implies
\begin{gather*}
\begin{aligned}
\dot{v}(t)&= \dot{x}(t) - G\dot{u}(t)\\
					&= {\Ah} x(t) - G\dot{u}(t)\\
          &= {\Ah}\big(v(t) + Gu(t)\big) - G\dot{u}(t)\\
          &= {\Ah}v(t) + {\Ah}Gu(t) - G\dot{u}(t)\\
          &= Av(t) + {\Ah}Gu(t) - G\dot{u}(t),
\end{aligned}
\end{gather*}
as $v(t) \in D(A)$ and \eqref{eq:BSC-ass1} holds.

Thus, if $x$ is a~classical solution of \eqref{eq:BCS}, then $v$ defined
by \eqref{eq:Book_11.7} is a~classical solution of \eqref{eq:Book_11.6}.
The other implication is proved similarly.
The uniqueness of the classical solutions of
\eqref{eq:BCS} follows from the uniqueness of a classical solution of
\eqref{eq:Book_11.6}.
\end{proof}	

The classical solution of \eqref{eq:Book_11.6} subject to every $v_0 \in D(A)$, every $u \in C^2([0,\tau],U)$ and any $\tau > 0$ is given by
\begin{equation}
v(t) = T(t)v_0 + \int_0^t T(t-r)\big({\Ah}Gu(r)-G\dot{u}(r)\big)dr.
\label{eq:Book_11.8}
\end{equation}
By means of a formula \eqref{eq:Book_11.7} we obtain for all $u \in C^2([0,\tau],U)$, all $x_0\in X$: $x_0 - Gu(0) \in D(A)$ and for all $\tau\geq 0$ the classical solution of \eqref{eq:BCS} in the form
\begin{equation}
\phi(t,x_0,u) = T(t)\big(x_0-Gu(0)\big)  + \int_0^t T(t-r)\big({\Ah}Gu(r)-G\dot{u}(r)\big) dr + Gu(t).
\label{eq:BCS-solution-for-smooth-inputs}
\end{equation}
Furthermore, the expression \eqref{eq:Book_11.8} is (by definition) a mild solution of \eqref{eq:Book_11.6} for every $v_0 \in X$ and every $u \in H^1([0,\tau],U)$, $\tau > 0$.

\mir{Explain, why do we consider $H^1$ space.
Actually, this space has to be defined (with values in $U$).

OK, does $u(0)$ make sense for $u \in H^1([0,\tau],U)$? If $U=\R$, then $u$ is absolutely continuous, and this does make sense.
}


Similarly, we define:
\begin{definition}
\label{def:Mild-solution-BCS} 
Therefore, the function
\begin{equation}
x(t) = T(t)(x_0-Gu(0))  + \int_0^t T(t-r)\big({\Ah}Gu(r)-G\dot{u}(r)\big) dr + Gu(t).
\label{eq:BCS-solution-for-smooth-inputs}
\end{equation}
is called the \emph{mild solution} of the abstract boundary control system 
\eqref{eq:BCS} for every $x_0 \in X$ and every $u \in H^1([0,\tau],U)$, $\tau > 0$.
\end{definition}


An advantage of the equation \eqref{eq:BCS-solution-for-smooth-inputs} is the boundedness of the operators $G$ and $\Ah G$, involved in the formula. The disadvantage of this solution formula is that it holds only for smooth inputs. We would like to derive another representation of the solutions of \eqref{eq:BCS}, which does not involve the derivatives of $u$.
To this end we apply the following result \cite[Corollary 10.1.4]{JaZ12}:
\begin{proposition}
\label{prop:Useful-formula} 
Let $T$ be a strongly continuous semigroup over a Banach space $X$ with the infinitesimal generator $A$.
Let also $f:\R_+\to X$ be so that $f(r) \in D(A)$ for all $r\geq 0$.
Then $\int_0^t T(t-r)f(r)dr \in D(A)$ for all $t\geq 0$ and the following holds:
\begin{eqnarray}
A\int_0^t T(t-r)f(r)dr = \int_0^t T(t-r)\dot{f}(r)dr + T(t)f(0) - f(t).
\label{eq:Generator_of_convolution}
\end{eqnarray}
\end{proposition}

\begin{proof}
\mir{The proof was not taken from \cite[Corollary 10.1.4]{JaZ12}.}

Pick any $h>0$, $t>0$ and consider the following expression:
{\allowdisplaybreaks
\begin{eqnarray}
\frac{T(h) - I}{h}\int_0^t T(t-r)f(r)dr 
&=& \frac{1}{h} \Big[\int_0^t T(h) T(t-r)f(r)dr - \int_0^t T(t-r)f(r)dr \Big] \nonumber\\
&=& \frac{1}{h} \Big[\int_0^t T(t+h-r)f(r)dr - \int_0^t T(t-r)f(r)dr \Big] \nonumber\\
&=& \frac{1}{h} \Big[\int_{-h}^{t-h} T(t-r)f(r+h)dr - \int_0^t T(t-r)f(r)dr \Big] \nonumber\\
&=& \frac{1}{h} \Big[\int_{-h}^{0} T(t-r)f(r+h)dr +  \int_{0}^{t-h} T(t-r)f(r+h)dr\nonumber\\
&&\qquad - \int_0^{t-h} T(t-r)f(r)dr - \int_{t-h}^t T(t-r)f(r)dr \Big] \nonumber\\
&=& \frac{1}{h}\int_{-h}^{0} T(t-r)f(r+h)dr - \frac{1}{h}\int_{t-h}^t T(t-r)f(r)dr \nonumber\\
&&  + \int_{0}^{t-h} T(t-r)\frac{f(r+h)-f(r)}{h}dr.
\label{eq:Computations-1}
\end{eqnarray}
}

Consider the first integral term in the previous expression:
\begin{eqnarray}
\frac{1}{h} \int_{-h}^{0} T(t-r)f(r+h)dr  
&=&  \frac{1}{h} \int_{-h}^{0} T(t-r)\big(f(r+h)-f(0)\big)dr \nonumber\\
&&\qquad\qquad+ \frac{1}{h} \int_{-h}^{0} T(t-r)f(0)dr. 
\label{eq:Term1.1}
\end{eqnarray}

Assume that $h<1$.
The first term of this expression can be easily estimated as follows:
\begin{eqnarray*}
 \Big\|\frac{1}{h} \int_{-h}^{0} T(t-r)\big(f(r+h)-f(0)\big)dr \Big\|_X 
&\leq&  \frac{1}{h} \int_{-h}^{0} \|T(t-r)\| \|f(r+h)-f(0)\|_X dr \\
&\leq&  M \sup_{r\in[-h,0]}\|f(r+h)-f(0)\|_X,
\end{eqnarray*}
where $M$ is so that $\|T(r)\|\leq M$ for all $r\in [0,1]$.
As $f$ is uniformly continuous on $[0,1]$, the last expression tends to zero as $h\to + 0$.

Furthermore,
\begin{eqnarray*}
\frac{1}{h} \int_{-h}^{0} T(t-r)f(0)dr
&=& T(t) \cdot \frac{1}{h} \int_{-h}^{0} T(-r)f(0)dr \\
&=& -T(t) \cdot \frac{1}{h} \int_{h}^{0} T(r)f(0)dr\\
&=& T(t) \frac{1}{h} \int_{0}^{h} T(r)f(0) - f(0)dr + T(t)f(0).
%\label{eq:}
\end{eqnarray*}
From the strong continuity of $T$ it follows that $\frac{1}{h} \int_{0}^{h} T(r)f(0) - f(0)dr \to 0$ as $h\to +0$, and we obtain from \eqref{eq:Term1.1}, that 
\begin{eqnarray}
\frac{1}{h} \int_{-h}^{0} T(t-r)f(r+h)dr  \to T(t)f(0),\qquad h\to +0.
\label{eq:Semigroup-formula-Integral-1}
\end{eqnarray}

Analogously, one can show that 
\begin{eqnarray}
\frac{1}{h} \int_{t-h}^t T(t-r)f(r)dr \to f(t),\quad h\to +0. 
%\frac{1}{h}\int_{t-h}^t T(t-r)(f(r)-f(t))dr + \frac{1}{h}\int_{t-h}^t T(t-r)f(t) dr \to f(t),\quad h\to 0. 
\label{eq:Semigroup-formula-Integral-2}
\end{eqnarray}
Finally, let us consider the last term in \eqref{eq:Computations-1}. We have that 

\mir{Add the explanations for the next formula}
\begin{eqnarray}
\lim_{h\to +0}\int_{0}^{t-h} T(t-r)\frac{f(r+h)-f(r)}{h}dr = \int_0^t T(t-r)\dot{f}(r)dr, 
\label{eq:Semigroup-formula-Integral-3}
\end{eqnarray}
and using \eqref{eq:Semigroup-formula-Integral-1}, \eqref{eq:Semigroup-formula-Integral-2}, \eqref{eq:Semigroup-formula-Integral-3} in \eqref{eq:Computations-1} we obtain the claim of the lemma.
\end{proof}

Using \eqref{eq:Generator_of_convolution} for the integral term in \eqref{eq:BCS-solution-for-smooth-inputs}, we obtain
another representation of the classical solution of \eqref{eq:BCS}.
\begin{eqnarray*}
%\label{eq:solution-formula-for-x-1}
x(t) 
&=& T(t)(x_0-Gu(0))  + \int_0^t T(t-r)\big({\Ah}Gu(r)-G\dot{u}(r)\big) dr + Gu(t)\\%\nonumber\\
&=& T(t)x_0 + \int_0^t T(t-r){\Ah}Gu(r)dr - \Big( \int_0^t T(t-r)G\dot{u}(r) dr + T(t)Gu(0) - Gu(t)\Big).
%&=& T(t)x_0 + \int_0^t T(t-r){\Ah}Gu(r)dr - A\int_0^t T(t-r)Gu(r) dr\nonumber\\
%&=& T(t)x_0 + \int_0^t T(t-r)({\Ah}G-AG)u(r)dr,
\end{eqnarray*}
Note that $G$ maps $U$ into $X$ (and not to $D(A)$), and thus $G\dot{u}(r)\in X$, $r\in[0,t]$ and in order to apply the formula \eqref{eq:Generator_of_convolution}, we need to lift the semigroup $T$ and its generator $A$ to space $X_{-1}$. These extensions we denote $T_{-1}$ and $A_{-1}$ respectively.

Then for $x_0 \in X$ and all $u\in C^2(\R_+,U)$ we obtain the following representation for the classical solution of \eqref{eq:BCS}:
\begin{eqnarray}
x(t) 
&=& T(t)x_0 + \int_0^t T_{-1}(t-r){\Ah}Gu(r)dr - A_{-1}\int_0^t T_{-1}(t-r)Gu(r) dr\nonumber\\
&=& T(t)x_0 + \int_0^t T_{-1}(t-r)({\Ah}G - A_{-1}G)u(r)dr,
\label{eq:solution-formula-for-x}
\end{eqnarray}
As we know from Theorem~\ref{thm:Fattorini-trick}, for $x_0 \in X$ and all $u\in C^2(\R_+,U)$ the solution of \eqref{eq:BCS} belongs to $X$,
in spite of the fact that what we integrate in \eqref{eq:solution-formula-for-x} is in $X_{-1}$.
However, the formula \eqref{eq:solution-formula-for-x} defining the function $x:\R_+ \to X_{-1}$ makes sense for all $x_0\in X$, all $t\geq 0$ and all $u\in L_{1,loc}(\R_+,U)$, and it defines a mild solution (in the space $X_{-1}$) of the equation 
\begin{eqnarray}
\dot{x} = A_{-1}x + ({\Ah}G-A_{-1}G)u.
\label{eq:BCS:State-space-representation}
\end{eqnarray}
corresponding to the initial condition $x(0)=x_0 \in X$.
However, for general nonsmooth $u$ we know only that the values of solutions lie in $X_{-1}$, and there is no guarantee that the solution lies in $X$. In order to ensure this, we have to require that the input operator 
\begin{eqnarray}
B:={\Ah}G-A_{-1}G
\label{eq:BCS-Input-Operator}
\end{eqnarray}
has some sort of admissibility. 

\begin{definition}
\label{def:Mild-solution-for-Boundary-Control-System} 
If $B$ defined by \eqref{eq:BCS-Input-Operator} is $q$-admissible, then for each $x_0\in X$ and each $u\in L_q(\R_+,U)$
the function $x:\R_+\to X$, defined by \eqref{eq:solution-formula-for-x} is called the mild solution of BCS \eqref{eq:BCS}.
\end{definition}

Note that uniqueness of the mild solution follows by uniqueness of a mild solution for the state space representation 
\eqref{eq:BCS:State-space-representation}.

\begin{remark}
\label{rem:Computation-of-B} 
Although the formula \eqref{eq:BCS-Input-Operator} gives us a general way to construct an input operator $B$, it may be awkward to use this formula in practice. Other methods for the computation of $B$ can be used, see \cite[Section 10.1]{TuW09}, and \cite{EmT00}.
\end{remark}



\subsection{Input-to-state stability of boundary control systems}
\label{sec:ISS-of-BSC}

Having the representations \eqref{eq:BCS-solution-for-smooth-inputs} (for smooth inputs) and \eqref{eq:BCS:State-space-representation} (for general inputs) for solutions of BCS \eqref{eq:BCS},
we can apply the criteria for ISS of  general linear systems for ISS analysis of BCS.
\begin{corollary}
\label{cor:ISS-for-BCS} 
Consider a boundary control system \eqref{eq:BCS} and assume that the corresponding input operator $B$ defined by 
\eqref{eq:BCS-Input-Operator} is $q$-admissible for some $q\in [1,+\infty)$. Assume that $A$ generates an exponentially stable semigroup
Then for any $p\in[q,+\infty]$
the system $\Sigma:=(X,\Uc,\phi)$ with $\Uc:=L_q(\R_+,U)$ is an ISS control system (with respect to norm in $\Uc$).
\end{corollary}

\begin{proof}
$B$ defined by \eqref{eq:BCS-Input-Operator} is $q$-admissible for some $q\in [1,+\infty)$, then it is $p$-admissible for any $p\in[q,+\infty]$ and furthermore, the map $\phi$ is continuous w.r.t. time. 
Proposition~\ref{prop:q-admissibility-implies-continuity} $\Sigma:=(X,\Uc,\phi)$ with $\Uc:=L_p([0,\infty),U)$, for all $p\in[q,+\infty]$ is a forward-complete control system in the sense of Definition~\ref{Steurungssystem},
and by  Proposition~\ref{prop:ISS-Criterion-lin-sys-with-unbounded-operators} $\Sigma$ is ISS.
\end{proof}


Now we proceed to study of stability properties of boundary control systems.
First of all, using Theorem~\ref{thm:Fattorini-trick}, we can prove that all 0-UGAS boundary control systems are ISS with respect to the inputs and their derivatives.


\mir{One should choose nice input spaces so that the derivative of the input exists and is again in a nice space.}


\begin{definition}
\label{def:D1-ISS} 
Let $\Sigma:=(X,\Uc,\phi)$ be a control system, and let $\Uc:=H^1([0,\tau],U)$ for a certain normed linear space $U$.
We call $\Sigma$ $D^1$-ISS, if there are $\beta\in\KL$ and $\gamma_0,\gamma_1\in\K$ so that 
for all $x\in X$, all $u\in\Uc$ and $t\geq 0$ it holds that
\begin{eqnarray}
\|\phi(t,x,u\|_X\leq \beta(\|x\|_X,t) + \gamma_0(\|u\|_\Uc) + \gamma_1(\|\dot{u}\|_\Uc).
\label{eq:D1-ISS}
\end{eqnarray}
\end{definition}



\subsection{Example}
\label{sec:Example}

As an example, consider the following linear heat equation.
\begin{eqnarray}
x_t(t,z) = \mu x_{zz}(t,z)
\label{eq:Linear_Diffusion-Dirichlet-control}
\end{eqnarray}
with a Dirichlet boundary input $u$:
\begin{eqnarray}
x(t,0)&=& 0 ,\quad t>0\\
x(t,1)&=& u(t), \quad t>0.
\label{eq:DirichletConditions_Linear_Diffusion-Dirichlet}
\end{eqnarray}
We assume that $X:=L_2(0,1)$ and $\Uc:=PC(\R_+,\R)$.

\mir{I am not sure that $\Uc:=PC(\R_+,\R)$ is a good choice. I have to go for more general input spaces.}

Interpreting $x(t,z)$ as the temperature of a body in a position $z\in[0,1]$ at time $t\geq 0$, the sense of the boundary condition \eqref{eq:DirichletConditions_Linear_Diffusion} is that at the end $z=0$ the zero temperature is maintained, and at the end $z=1$ we can regulate the temperature by means of a control $u$.

This system can be naturally written in the form \eqref{eq:BCS}
where:
\begin{itemize}
	\item the formal system operator $\Ah$ is given by
	\begin{eqnarray}
	\Ah x= \frac{d^2 x}{dx^2},\quad x \in D(\Ah) := H^2(0,1) \cap H^1_L(0,1),
	\label{eq:Formal-system-operator-Heat}
	\end{eqnarray}
	with 
	\begin{eqnarray}
	H^1_L(0,1) := \{g\in H^1(0,1): g(0)=0\}.
	\label{eq:H1L-definition}
	\end{eqnarray}

	\item The \emph{boundary operator} $\Gh:X \to \R$ is given by 
	\begin{eqnarray}
	\Gh (x) = x(1),\quad x \in D(\Gh) := H^2(0,1) \cap H^1_L(0,1),
	\label{eq:Boundary-opertator-Heat}
\end{eqnarray}

	\item $u(t) \in \R$
\end{itemize}

Before we analyze the general case let us see how this works in the case of systems \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}, 
\eqref{eq:Linear_Diffusion-Dirichlet-control}.

Assume that $u$ is a continuously differentiable input and that $x$ is a corresponding classical solution of a system 
\eqref{eq:Linear_Diffusion-Dirichlet-control}, \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}.
Define
\begin{equation*}
v(z, t) = x(z, t) - z u(t),\quad z\in[0,1],\ t\geq 0.
\end{equation*}
We obtain the following partial differential equation for $v$:
\begin{eqnarray*}
v_t(z, t) & =& v_{zz} (z, t) - z\dot{u}(t), \qquad z\in[0, 1], \quad t \geq0\\
v(0,t) &=& v(1, t) = 0,\quad t\geq0.
\end{eqnarray*}
This partial differential equation for $v$ is a system with a distributed control $\tilde{u} := \dot{u}$, which can be represented as an abstract evolution equation
\begin{equation*}
\dot{v}(t) = Av(t) + \tilde{B}\tilde{u}(t)
\end{equation*}
for a certain infinitesimal generator $A$ and a bounded operator $\tilde{B}$.
Thus, for smooth inputs a system 
\eqref{eq:Linear_Diffusion-Dirichlet-control}, \eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet}
with boundary inputs can be converted into the classical form \eqref{eq:BCS-standard-linear-systems}.
At the same time, one can show that the system \eqref{eq:Linear_Diffusion-Dirichlet-control},
\eqref{eq:DirichletConditions_Linear_Diffusion-Dirichlet} \emph{cannot} be written in a form \eqref{eq:BCS-standard-linear-systems} \emph{for all inputs in $\Uc$ with a bounded operator $B$}, see Exercise~\ref{ex:BCS-Transport-equation}, item (iii) for the same question for the transport equation.




\subsection{Input-to-state stability of boundary control systems}

\mir{$\phi(t,x,u)$ instead of $x(t)$.}

Theory of general boundary control systems has started its development with the pioneer work \cite{Fat68}, and it was greatly developed by \cite{Sal87}. In the literature there are several ways how to define a boundary control system, see e.g. \cite{Fat68}, \cite{CuZ95, JaZ12}, 
\cite{Sal87,TuW09} and \cite{EmT00}. The discussion of the differences between various methods is discussed e.g. in \cite{LGE00}.
We adopt here the definition of a boundary control system from \cite{JaZ12} and the method of deriving the state space representation for this kind of systems from \cite{EmT00}.


ISS of linear parabolic systems w.r.t. boundary disturbances has been studied in several recent papers using different methodologies \cite{AWP12, KaK16b, KaK17a, JNP18}.
In \cite{AWP12} the authors attacked this problem by means of Lyapunov methods. Due to the methodology followed in \cite{AWP12} boundary disturbances must be differentiated w.r.t. time (which is also needed when one tries to switch from boundary to distributed disturbances). As a result, in \cite{AWP12} ISS of a parabolic system w.r.t. $C^1$ norm has been achieved (known as $D^1$-ISS, see \cite[p. 190]{Son08}).

Similar ideas have been applied in \cite{AVP16} for much more complex systems as the Burgers' equation with nonlinear forcing and the Kuramoto-Sivashinsky equation.

In \cite{KaK16b, KaK17a, KaK17b} linear parabolic PDEs with Sturm-Liouville operators over 1-dimensional spatial domain have been treated by using two different methods: (i) the spectral decomposition of the solution, and (ii) the approximation of the solution by means of a  finite-difference scheme. 
This made possible to avoid differentiation of boundary disturbances, and to obtain ISS of classical solutions w.r.t. $L^\infty$ norm of disturbances, as well as in weighted $L^2$ and $L^1$ norms. 
An advantage of these methods is that this strategy can be applied also to other types of linear evolution PDEs. At the same time, for multidimensional spatial domains, the computations can become quite complicated.

In \cite{JNP18} ISS of linear boundary control systems has been approached by means of methods of semigroup and admissibility theory. In particular, interesting and nontrivial relations between ISS and integral input-to-state stability (iISS) have been obtained. 
An advantage of this method is that it encompasses very broad classes of linear infinite-dimensional systems, but due to the lack of proper generalizations of admissibility to general nonlinear systems, it cannot be applied (at least at current stage) to nonlinear distributed parameter systems.

In \cite{TPT16} it was shown that well-known constructions of Lyapunov functions for first order hyperbolic PDEs without inputs (for a survey see \cite{BaC16}) can serve also as ISS Lyapunov functions for wide classes of hyperbolic systems of the first order with inputs. These results have been applied in \cite{TPT16} to achieve an ISS stabilization of linear systems of conservation laws by means of boundary controllers which are subject to additive quantization errors.

In \cite{ZhZ18} constructions of ISS coercive Lyapunov functions for a class of nonlinear parabolic systems with Neumann or Robin boundary inputs have been presented. These results are very promising since before this work only non-Lyapunov methods have been exploited to study of such systems \cite{KaK16b, KaK17a, KaK17b, JNP18, MKK19}. The results in \cite{ZhZ18} have been obtained using novel Poincare-like integral inequalities for systems with boundary inputs. 
However, the methods used in \cite{ZhZ18} cannot be applied to systems with Dirichlet boundary inputs.


\todo{}

\subsection{Exercises}




\begin{exercise}
\label{ex:ex-BCS-1}
Consider a boundary control system as in Definition~\ref{def:BCS}.

Show that $x_0 - Gu(0) \in D(A)$ holds if and only if $x_0 \in D({\Ah})$ and ${\Gh}x_0 = u(0)$.
\end{exercise}

\ifAndo
\begin{solution*}
'$\Rightarrow$'. Assume that $x_0 - Gu(0) \in D(A)$. Then also $x_0 - Gu(0) \in D({\Ah})$. 
By definition of a control system it holds that $G u(0) \in D({\Ah})$.
As $D({\Ah})$ is a linear space, $x_0 \in D({\Ah})$ as well.

As $D(A) = D({\Ah}) \cap \ker ({\Gh})$, it holds that 
\[
0 = {\Gh}(x_0-G u(0)) = {\Gh}x_0 - {\Gh}G u(0) = {\Gh}x_0 - u(0).
\]

'$\Leftarrow$'. Let $x_0 \in D({\Ah})$ and ${\Gh}x_0 = u(0)$.
We have that
\[
{\Gh}(x_0-G u(0)) = {\Gh}x_0 - {\Gh}G u(0) = {\Gh}x_0 - u(0) = 0.
\]
Furthermore, due to the definition of a boundary control system, it holds that $G u(0) \in D({\Ah})$, and as $D({\Ah})$ is a linear space, also $x_0 - Gu(0) \in D({\Ah})$.
As $D(A) = D({\Ah}) \cap \ker ({\Gh})$, this shows the claim of the lemma. 
\hfill$\square$
\end{solution*}
\fi


\begin{exercise}
\label{ex:Finishing-proof-of-Theorem-Fattorini-Trick}
Show the converse implication in Theorem~\ref{thm:Fattorini-trick}. 
\end{exercise}

\ifAndo
\begin{solution*}
Assume that $v$ is a~classical solution of \eqref{eq:Book_11.6}.
Then for $t \in [0, \tau]$ we obtain 
$v(t) \in D(A) \subset D({\Ah}) \subset D({\Gh})$,
$Gu(t) \in D({\Gh})$, and
since
$v(t) \in D(A) \subset \ker{\Gh}$ and
the equation \eqref{eq:BSC-ass2} holds, we obtain that
\begin{equation*}
{\Gh}x(t) = {\Gh}(v(t) + Gu(t))
 = {\Gh}v(t) +{\Gh}Gu(t) = u(t).
\end{equation*}
Furthermore, equation \eqref{eq:Book_11.7} implies
\begin{gather*}
\begin{aligned}
\dot{x}(t)&= \dot{v}(t) + G\dot{u}(t)
\\
          &= Av(t) - G\dot{u}(t)
           + {\Ah}Gu(t) + G\dot{u}(t) \qquad && \text{by \eqref{eq:Book_11.6}}
\\
          &= Av(t) + {\Ah}Gu(t)
\\
          &= {\Ah}(v(t) + Gu(t))             && \text{by \eqref{eq:BSC-ass1}}
\\
          &= {\Ah}x(t)                       && \text{by \eqref{eq:Book_11.7}}.
\end{aligned}
\end{gather*}
Thus, if $v$ is a~classical solution of \eqref{eq:Book_11.6}, then $x$ defined
by \eqref{eq:Book_11.7} is a~classical solution of \eqref{eq:BCS}.

The other implication is proved similarly.
The uniqueness of the classical solutions of
\eqref{eq:BCS} follows from the uniqueness of the classical solutions of
\eqref{eq:Book_11.6}, see Theorem 10.1.3. 
\hfill$\square$
\end{solution*}
\fi


\begin{exercise}
\label{ex:BCS-Transport-equation}
Consider the controlled transport equation
\begin{gather*}
\begin{aligned}
\frac{\partial x}{\partial t}(z, t)
           &= \frac{\partial x}{\partial z}(z, t), \quad && z\in [0,1], \quad t\geq0
\\
x(z, 0)&= x_0(z),                                        && z\in [0, 1]
\\
     x(1,t)&= u(t),                                              && t\geq0
\end{aligned}
\end{gather*}
for an input $u \in H^1(0,\tau)$ and on the state space $X = L^2(0, 1)$.
Let us rewrite the transport equation in the following form:
\begin{gather*}
\begin{aligned}
{\Ah}x &= \frac{dx}{dz},  && D({\Ah})=H^1(0, 1),
\\
{\Gh}x &= x(1), \qquad        && D({\Gh})=D({\Ah}).
\end{aligned}
\end{gather*} 

\begin{itemize}
	\item[(i)] Show that these equations define a boundary control system. 
	\item[(ii)] Compute the solution of this system.
	\item[(iii)] Show that this equation cannot be written in the form 
\eqref{eq:BCS-standard-linear-systems} with a bounded operator $B$ and any infinitesimal generator $A$.
\end{itemize}
\end{exercise}


\ifAndo
\begin{solution*}
{\color{red} The solution is taken from \cite{JaZ12}.}

\begin{itemize}
	\item[(i)] These two operators satisfy
the assumption of a~boundary control system.
More precisely: the
operators ${\Ah}$ and ${\Gh}$ are linear,
${\Ah}$~restricted to the domain $D({\Ah})\cap\ker{\Gh}$
generates a~$C_0$-semigroup, see Exercise {6.3}.
Furthermore, the range
of ${\Gh}$ is $\mathbb{C}=U$
and the choice $G = \mathds{1}_{[0,1]}$ implies
${\Gh}Gu = u$.

	\item[(ii)]
	Using the fact that ${\Ah}G = 0$,
we conclude from equation \eqref{eq:BCS-solution-for-smooth-inputs} that the mild
solution is given by
\begin{gather*}
\begin{aligned}
x(t) & = T(t)(x_0-Gu(0))
        + \int_0^t T(t-s)({\Ah}Gu(s)-G\dot{u}(s)) ds + Gu(t)
\\
     & = T(t)(x_0-u(0))-\int_0^t T(t-s)\mathds{1}_{[0,1]}\dot{u}(s) ds + u(t).
\end{aligned}
\end{gather*}
Using the precise representation of the
shift-semigroup, see Exercise {6.3}, we can write the solution of the
boundary controlled partial differential equation as
\begin{gather*}
x(z, t) = (x_0(z + t)-u(0))\mathds{1}_{[0,1]}(z + t)
 - \int_0^t \mathds{1}_{[0,1]}(z + t-s)\dot{u}(s) ds + u(t).
\end{gather*}
If $z + t > 1$, we have
\begin{gather*}
x(z, t) = -u(\tau)\Big|_{z+t-1}^t + u(t) = u(z + t-1),
\end{gather*}
and if $z + t \leq 1$, then
\begin{gather*}
x(z, t) = x_0(z + t)-u(0)-u(\tau)\Big|_0^t
 = x_0(z + t).
\end{gather*}
Or equivalently,
\begin{equation}
x(z, t) =
\begin{cases}
    x_0(z + t), & z + t \leq 1,
    \\
    u(z + t-1), & z + t > 1,
\end{cases}
\label{eq:Book_11.10}
\end{equation}

	\item[(iii)]
If the controlled transport equation were of the form \eqref{eq:BCS-standard-linear-systems},
then {\color{red} Theorem ??? (add references)}
would imply that $x(t) \in D(A)$, whenever $x(0) \in D(A)$
and $u \in C^1([0,\tau];X)$.
Choosing $x_0 = 0$, $t = \frac{1}{2}$, and $u=1$, \eqref{eq:Book_11.10}
implies that
$x(z, \frac{1}{2}) = 0$ if $z\leq\frac{1}{2}$
and $x(z, \frac{1}{2}) = 1$ if $z > \frac{1}{2}$, which is
in contradiction to $x(\frac{1}{2}) \in D(A) \subset D({\Ah}) = H^1(0,1)$.
Summarizing, the boundary controlled transport equation of this
example cannot be written in the form \eqref{eq:BCS-standard-linear-systems}.
\end{itemize}
\hfill$\square$
\end{solution*}
\fi




\subsection{Reading plan}


\begin{enumerate}
	\item Boundary control systems and ISS
	
	\begin{itemize}
		\item \cite{ScZ18}, see Section~\ref{sec:ScZ18}.
	This is a very clear overview of boundary control systems for nonlinear boundary controls.
	
	Also it is interesting to see the approximation theory of the weak or generalized solutions and classical solutions.
	
	First for the classical solutions the results are obtained and then by approximation the results for mild solutions are obtained.
	
		\item In a linear case the paper 'ISS Property with Respect to Boundary Disturbances for a Class of Riesz-Spectral Boundary Control Systems'
is of value.
Here a nice overview of the method of the spectral decomposition has been performed and again the ideas of the approximation of the mild solutions via classical solutions is used. 

One more paper with the similar approach is 
'Input-to-State Stability of a Clamped-Free Damped String in the Presence of Distributed and Boundary Disturbances'

		\item It makes sense to look at \cite{JaZ12} for the overview of the boundary control systems in order to understand the basics.
		\item One of the questions is probably how the boundary control systems are related to the systems with the unbounded input operators.
		Are boundary control systems always systems with admissible input operators?
		And how both these classes are related to the class of well-posed systems in the sense of Weiss and Tuscnak (or in the sense of Staffans)?
		
	\end{itemize}
	
	\item Well-posedness for systems with boundary controls
	
	As I understand, one of the possibilities is to show that this is a boundary control systems.
	But it seems that there were also other ways, see the paper 'Input-to-State Stability of an ODE-heat
Cascade System with Disturbances'.

It seems, that Hans Zwart started to work on that: how to show well-posedness of the nonlinear boundary control systems.

	\item Nonlinear PDEs with a linear boundary control operator.
	Papers by Jun and coauthors.
	
	\item Nice applications in papers by Iasson and Miroslav.


\item Read Appendix D in ISEM 2012-2013 on weak derivatives and Sobolev spaces.

\item Evans, semigroup theory
Chapter on Evolution equations in Banach spaces
	
\end{enumerate}


\subsection{On boundary control systems}

As I understand, for smooth inputs boundary control systems have continuously differentiable classical solutions.
Moreover, for the mild data, i.e. $(x,u) \in X\tm H^1([0,\tau],U)$ these systems still have continuous solutions.

Thus the question: do these systems possess all the properties of control systems as in \cite{MiW18b}?

Furthermore, port-Hamiltonian systems are a special case (at least under reasonable assumptions) of boundary control systems,
see \cite[Section 11.3]{JaZ12}.

There is a generalization of port-Hamiltonian system, when instead of  $P_0^T+P_0 = 0$ a condition $P_0^T+P_0 \leq 0$ is satisfied.
Such systems may be called port-dissipative systems, see \cite{Sch18}.


For the survey
\begin{itemize}
	\item Define boundary-control systems
	\item Under which conditions do the BCS satisfy the axioms which we have in MiW18b?
	\item Port-Hamiltonian systems (or maybe port-dissipative systems) as BCS.
	\item Well-posedness.
\end{itemize}
Probably I should write something about port-Hamiltonian systems



\subsection{Ideas about \cite{Sch18} paper.}
\label{sec:Sch18}

Jochen has several nice examples and counterexamples on relations between AG, sAG and UAG properties.
They can be included to the book on ISS as examples or as exercises.
In particular, modulated linear systems is an interesting class of systems.




\subsection{Ideas about \cite{LSZ18} paper.}
\label{sec:LSZ18}

The paper \cite{LSZ18} is quite interesting, as it shows how the strategy with decomposition of systems in modes can be used in pratice, and how the well-posedness of the systems can be analyzed.

Basically, 
\begin{itemize}
	\item First one shows that the operator generates a contraction semigroup by Lumer-Phillips. Dissipativity is first checked. Then one directly computes the inverse operator, shows its boundedness and in this way shows that it is surjective.
	
	Actually, if we get merely boundedness of the inverse on the dense domain (and thus existence of an extension of the inverse to the whole domain), does this imply the surjectivity of an operator?
	
	\item Afterwards, they show that the system is a boundary control system and infer from this that the system is well-posed. This should be checked.
	
	\item Afterwards, they study the spectral properties of an operator, and derive the Riesz basis.
	
	\item It is verified that the operator under consideration is a Riesz-spectral operator.
	
	\item Finally, they decompose the state w.r.t. the Riesz basis and derive equations for the individual modes.
	Then ISS of the modes is analyzed and finally ISS of the whole system is derived.
\end{itemize}
There are many interesting explanations in the paper, and it is easy to read, although I have not checked all the derivations.



\subsection{Ideas about \cite{ScZ18} paper.}
\label{sec:ScZ18}


In this paper the authors consider the stabilization of port-Hamiltonian systems via nonlinear boundary controls.
These controllers are subject to external disturbances, and thus even robust stabilization in ISS or weak ISS sense respectively is acheived.
The authors do not design a particular controller but rather identify a class of controllers which are allowed to achieve ISS or weak ISS of a closed-loop system. 



\section{Linear systems}
\label{sec:LinSys}

In this section, we derive (coercive as well as non-coercive) converse ISS Lyapunov theorems for linear systems with a
bounded input operator $B$ of the form
\begin{equation}
\label{LinSys}
\dot{x}=Ax+Bu.
\end{equation}
The assumptions on $A$ are as before and we continue to consider $\Uc:=PC_b(\R_+,U)$.

In contrast to the results for nonlinear systems from the previous sections, for linear systems with bounded input operators,
ISS Lyapunov functions can be constructed in a more explicit form. We start with a definition.
\begin{definition}
System \eqref{InfiniteDim} is {\it globally asymptotically
stable at zero uniformly with respect to the state} (0-UGAS), if there
exists a $ \beta \in \KL$, such that
\begin{equation}
\label{UniStabAbschaetzung}
x \in X,\ t \geq 0 \quad \Rightarrow \quad \left\| \phi(t,x,0) \right\|_{X} \leq  \beta(\left\| x \right\|_{X},t) .
\end{equation}
\end{definition}

Now we proceed with a technical lemma; its proof is straightforward and is omitted.
\begin{lemma}
\label{AuxiliaryEquality}
Let $B \in L(U,X)$ and let $T$ be a $C_0$-semigroup. Then for any $u\in
{\cal U}$ it holds that
\begin{eqnarray}
\lim\limits_{h \rightarrow +0} \frac{1}{h} \int_0^h{T_{h-s} B u(s)ds} = B u(0).
\label{eq:Convolution_Bu0}
\end{eqnarray}
\end{lemma}

Theorem~\ref{ISS_Converse_Lyapunov_Theorem} shows that ISS is equivalent to the existence of a Lipschitz continuous \textit{coercive ISS Lyapunov function}. 
Nevertheless, it is well-known, that Lyapunov functions for linear infinite-dimensional systems, constructed by solving an operator Lyapunov equation, are in general non-coercive (see \cite[Theorem 5.1.3]{CuZ95}).
\ifSCL%
\else This is one of the reasons making non-coercive Lyapunov functions very natural for infinite-dimensional systems.
\fi
We now show that such Lyapunov functions are in fact \textit{non-coercive ISS Lyapunov functions for any bounded input operator $B$}. 

\begin{proposition}
\label{ConverseLyapunovTheorem_LinearSystems}
If \eqref{LinSys} is 0-UGAS, then $V:X \to \R_+$, defined as
\begin{eqnarray}
V(x)=\int_0^{\infty} \|T_t x\|_X^2 dt
\label{eq:LF_LinSys_Banach}
\end{eqnarray}
is a non-coercive ISS Lyapunov function for \eqref{LinSys} which is
locally Lipschitz continuous.
 Moreover, for all $ x \in X$, $ u \in {\cal U}$ and $ \eps>0$ it holds that 
\begin{equation}
\label{Final_Lyapunov_Inequality}
\dot{V}_u(x) \leq -\|x\|_X^2 + \frac{\eps M^2}{2\lambda} \|x\|_X^2 + \frac{M^2}{2\lambda \eps}  \|B\|^2 \|u(0)\|_U^2,
\end{equation}
where $M, \lambda>0$ are so that 
\begin{equation}
\|T_t \| \leq M e^{-\lambda t}.
\label{eq:SemigroupEstimate}
\end{equation}
\end{proposition}

\begin{proof}
Let \eqref{LinSys} be 0-UGAS and pick $u\equiv 0$. 
Then \eqref{UniStabAbschaetzung} implies $\|T_t x\|_X \leq \beta(1,t)$ for
all $t \geq 0$ and for all $x$ with  $\|x\|_X=1$. Since $\beta \in \KL$,
there exists a $t^*$ such that  $\|T_{t^*}x\|_X < 1$ for all $x \in X$:
$\|x\|_X=1$. Thus, $\|T_{t^*}\|<1$ and consequently $T$ is an exponentially
stable semigroup \cite[Theorem 2.1.6]{CuZ95}, i.e. there exist
$M,\lambda>0$ such that \eqref{eq:SemigroupEstimate} holds.

Consider $V:X \to \R_+$ as defined in \eqref{eq:LF_LinSys_Banach}.
We have
\begin{eqnarray}
V(x) \leq \int_0^{\infty}\hspace{-1.5mm} \|T_t \|^2\|x\|_X^2 dt \leq \frac{M^2}{2\lambda} \|x\|_X^2.
\label{eq:LF_Upper_estimate}
\end{eqnarray}

Let $V(x)=0$. Then $\|T_t x\|_X \equiv 0$ a.e. on $[0,\infty)$. Strong continuity of $T$ implies that $x = 0$, and thus 
\eqref{LyapFunk_1Eig_noncoercive} holds.

Next we estimate the Dini derivative of $V$: 
{\allowdisplaybreaks
\begin{align*}
\dot{V}_u(x)& = \mathop{\overline{\lim}} \limits_{h \rightarrow +0} {\frac{1}{h}(V(\phi(h,x,u))-V(x)) } \\
    = & \mathop{\overline{\lim}} \limits_{h \rightarrow +0} {\frac{1}{h}\Big(\int_0^{\infty} \|T_t \phi(h,x,u)\|_X^2 dt - \int_0^{\infty} \|T_t x\|_X^2 dt \Big) } \\
\ifSCL
\else    = & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}
\frac{1}{h}\Big(\int_0^{\infty} \Big\|T_t \Big(T_hx + \int_0^h{T_{h-s} B
  u(s)ds}\Big) \Big\|_X^2 dt \\
    & \quad -\int_0^{\infty} \|T_t x\|_X^2 dt \Big)  \\
\fi
    = & \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \frac{1}{h}\Big(\int_0^{\infty} \Big\|T_{t+h} x + T_t \int_0^h{T_{h-s} B u(s)ds}\Big\|_X^2 dt \\
		    & \quad - \int_0^{\infty} \|T_t x\|_X^2 dt \Big) \\  
   \leq & \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \frac{1}{h}\Big(\int_0^{\infty} \Big(\Big\|T_{t+h} x\Big\|_X \\
    &\quad + \Big\|T_t \int_0^h\hspace{-1.5mm}{T_{h-s} B u(s)ds}\Big\|_X \Big)^2 dt - \int_0^{\infty} \hspace{-1.5mm}\|T_t x\|_X^2 dt \Big)  \\
   = & I_1 + I_2,
\end{align*}
}
where $I_1:= \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \frac{1}{h}\Big(\int_0^{\infty} \|T_{t+h} x\|_X^2 dt - \int_0^{\infty} \|T_t x\|_X^2 dt \Big)$,
\begin{align*}
\text{and}\ \ I_2  := &\mathop{\overline{\lim}} \limits_{h \rightarrow +0} \frac{1}{h}  \int_0^{\infty} \Big( 2\Big\|T_{t+h} x\Big\|_X \Big\|T_t \int_0^h\hspace{-1.5mm}{T_{h-s} B u(s)ds}\Big\|_X \\
 &\quad\quad\quad\quad + \Big\|T_t \int_0^h{T_{h-s} B u(s)ds}\Big\|_X^2 \Big) dt.
%\label{eq:I2}
\end{align*}
\ifSCL
We have: $I_1 = \mathop{\overline{\lim}} \limits_{h \rightarrow +0} - \frac{1}{h}   \int_0^h \|T_t x\|_X^2 dt 
    = -\|x\|_X^2.$
\else
Let us compute $I_1$:
\begin{align*}
I_1 
&= \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \frac{1}{h}\Big(   \int_h^{\infty} \|T_t x\|_X^2 dt - \int_0^{\infty} \|T_t x\|_X^2 dt \Big) \\
    &= \mathop{\overline{\lim}} \limits_{h \rightarrow +0} - \frac{1}{h}   \int_0^h \|T_t x\|_X^2 dt 
    = -\|x\|_X^2.
\end{align*}
\fi

Now we proceed with $I_2$:
\begin{align*}
I_2 \leq & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}  \int_0^{\infty}\hspace{-1.5mm} 2\Big\|T_{t+h} x\Big\|_X \Big\|T_t \frac{1}{h} \int_0^h\hspace{-1.5mm}{T_{h-s} B u(s)ds}\Big\|_X dt \\
      & \qquad\qquad+ \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \int_0^{\infty}\hspace{-1mm} \frac{1}{h} \Big\|T_t \int_0^h{T_{h-s} B u(s)ds}\Big\|_X^2 dt.
\end{align*}
The limit of the second term equals zero since
\begin{align*}
\mathop{\overline{\lim}} \limits_{h \rightarrow +0} \int_0^{\infty}& \frac{1}{h} \Big\|T_t   \int_0^h{T_{h-s} B u(s)ds}\Big\|_X^2 dt \\
\leq \mathop{\overline{\lim}} \limits_{h \rightarrow +0} \int_0^{\infty} \frac{1}{h} M^4 e^{-2\lambda t}\|B\| \|u\|_{\cal U}
h^2 dt 
= \ 0.
\end{align*}
To compute the limit of the first term, note that 
\begin{align*}
2\Big\|T_{t+h} x\Big\|_X \Big\|T_t \frac{1}{h} & \int_0^h{T_{h-s} B u(s)ds}\Big\|_X \\
\leq&
2 M \|x\|_X \|T_t \| M  \|B\| \sup_{r \in [0,h]}\|u(r)\|_{U} \\
\leq&
2 M^3 \|x\|_X  \|B\| \|u\|_{\cal U} e^{-\lambda t}.
\end{align*}
Applying the dominated convergence theorem, Lemma~\ref{AuxiliaryEquality} and Young's inequality we obtain for any $\eps >0$ that
\begin{eqnarray*}
\hspace{-8mm}
I_2 & = & \int_0^{\infty} 2\|T_t x\|_X \|T_t  B u(0)\|_X dt \\
    & \leq & \int_0^{\infty} \eps \|T_t x\|_X^2 + \frac{1}{\eps} \|T_t  B u(0)\|_X^2 dt \\
\ifSCL
\else    & \leq & \int_0^{\infty} \eps \|T_t \|^2 dt \|x\|_X^2 + \frac{1}{\eps} \int_0^{\infty} \|T_t \|^2 \|B u(0)\|_X^2 dt \\
\fi    
  & \leq &  \frac{\eps M^2}{2\lambda} \|x\|_X^2 + \frac{M^2}{2\lambda \eps}  \|B\|^2 \|u(0)\|_U^2.
\end{eqnarray*}
Overall, we obtain that  $\forall x \in X$, $\forall u \in {\cal U}$ and for all $\eps>0$ the inequality \eqref{Final_Lyapunov_Inequality} holds. Considering $\eps < \frac{2\lambda}{M^2}$ this shows that $V$ is a non-coercive ISS Lyapunov function (in dissipative form) for \eqref{LinSys}.
It can be brought into implication form (as in \eqref{DissipationIneq}) by choosing the Lyapunov gain $\chi(s):=Rs$ for all $s \in \R_+$ and for $R$ large enough.

It remains to show the local Lipschitz continuity of $V$.
\ifSCL We omit the straightforward computations.
\else
Pick arbitrary $r>0$ and any $x,y \in \overline{B}_r$. It holds that
\begin{align*}
|V&(x) - V(y)| = \Bigg| \int_0^{+\infty} \|T_t x\|^2_X - \|T_t y\|^2_X dt \Bigg| \\
&\leq   \int_0^{+\infty} \Big|\|T_t x\|_X - \|T_t y\|_X\Big| \big(\|T_t x\|_X + \|T_t y\|_X\big) dt \\
&\leq   \int_0^{+\infty} \|T_t x - T_t y\|_X \big(\|T_t x\|_X + \|T_t y\|_X\big) dt \\
&\leq   \int_0^{+\infty} Me^{-\lambda t} \|x - y\|_X Me^{-\lambda t} (\|x\|_X + \|y\|_X) dt \\
&\leq   \frac{M^2 r}{\lambda} \|x-y\|_X,
\end{align*}
which shows the Lipschitz continuity of $V$.
\fi
\end{proof}

\begin{remark}
The ISS Lyapunov function
$V$ defined in \eqref{eq:LF_LinSys_Banach} is not coercive in general. 
Noncoercivity of $V$ defined by \eqref{eq:LF_LinSys_Banach} implies that the system
\[\dot{x}=Ax, \quad y=x\]
is not exactly observable on $[0,+\infty)$ (even though we can measure the full state!), see \cite[Corollary 4.1.14]{CuZ95}.
The reason for this is that for any given exponential decay rate there are
states decaying at a faster rate, and thus part of the information about
the state disappears "infinitely fast".
%Under the additional assumption that
%\begin{eqnarray}
%\|T_t x\|_X \geq M_2 e^{-\lambda_2 t} \|x\|_X
%\label{eq:T_coercivity}
%\end{eqnarray}
%for some $M_2,\lambda_2>0$ and for all $x \in X$,
%$V$ defined in \eqref{eq:LF_LinSys_Banach} is a coercive ISS-Lyapunov function for \eqref{LinSys}, since
%\begin{eqnarray}
%V(x) \geq \alpha_1  \|x\|_X^2
%\label{eq:Est_from_below}
%\end{eqnarray}
%holds for some $\alpha_1>0$. 
\end{remark}

\begin{remark}
\label{rem:Non-coercive_ISS_LFs} 
Note that according to \cite[Section III.B]{MiW18b}, the existence of a non-coercive Lyapunov function satisfying 
\eqref{Final_Lyapunov_Inequality} ensures ISS of
\eqref{LinSys}.
\end{remark}


%%%%%%%
Below we provide another construction of ISS Lyapunov functions for the system \eqref{LinSys} with bounded input operators.
It is based on a standard construction in the analysis of $C_0$-semigroups, see e.g. \cite[Eq. (5.14)]{Paz83}.

For exponentially stable $C_0$-semigroup $T$ there exist $M,\lambda>0$ such that the estimate
\eqref{eq:SemigroupEstimate} holds. Choose $\gamma>0$ such that $\gamma -
\lambda < 0$. Then
\begin{equation}
    \label{eq:eqnorm}
    V^\gamma (x) := \max_{s\geq 0} \| e^{\gamma s} T_s x\|_X
\end{equation}
defines an equivalent norm on $X$, for which we have
\begin{align}
    \label{eq:eqnorm2}
    V^\gamma(T_t x) 
\ifSCL 
\else = \max_{s\geq 0} \| e^{\gamma s} T_s T_t  x\|_X \\ 
\fi
&=
    e^{-\gamma t} \max_{s\geq 0} \| e^{\gamma (s+t)} T_{s+t} x\|_X {\leq}
    e^{-\gamma t} V^\gamma(x) \,.
\end{align}
Based on this inequality we obtain the following statement for ISS
Lyapunov functions.

\begin{proposition}
    \label{p:Lyapunovfunction2}
    Let \eqref{LinSys} be 0-UGAS. Let $M,\lambda>0$ be such that
\eqref{eq:SemigroupEstimate} holds and let $0<\gamma < \lambda$.
Then $V^\gamma :X \to \R_+$, defined by \eqref{eq:eqnorm}
is a coercive ISS Lyapunov function for \eqref{LinSys}. In particular, for
any $u\in {\cal U}$, $x\in X$, we
have the dissipation inequality
\begin{equation}
    \label{eq:dissipation2}
    \dot{V}^\gamma_u(x) \leq - \gamma \ V^\gamma(x) + V^\gamma (Bu(0)) \,.
\end{equation}
\end{proposition}

\begin{proof}
We start by showing Lipschitz continuity of $V^\gamma$. Pick any $x,y \in X$ and assume that
$V^\gamma(x) > V^\gamma(y)$.
Then
\begin{align*}
V^\gamma&(x) - V^\gamma(y) = \max_{s\geq 0} \| e^{\gamma s} T_s x\|_X - \max_{s\geq 0} \| e^{\gamma s} T_s y\|_X \\
& \leq \max_{s\geq 0} \big(\| e^{\gamma s} T_s x\|_X - \| e^{\gamma s} T_s y\|_X\big) \\        
& \leq \max_{s\geq 0} \big| \| e^{\gamma s} T_s x\|_X - \| e^{\gamma s} T_s y\|_X \big|\\
& \leq \max_{s\geq 0} \| e^{\gamma s} T_s(x-y)\|_X 
 \leq M\|x-y\|_X,        
\end{align*}
which shows that $V^\gamma$ is globally Lipschitz continuous. The case $V^\gamma(y) > V^\gamma(x)$ can be treated analogously.

In order to obtain an infinitesimal estimate, we compute, using the
    triangle inequality ($V^\gamma$ is a norm), the estimate
    \eqref{eq:eqnorm2}, and Lemma~\ref{AuxiliaryEquality},
{\allowdisplaybreaks		
    \begin{align*}
    \dot{V}^\gamma_u&(x) = \mathop{\overline{\lim}} \limits_{h \rightarrow +0} {\frac{1}{h}(V^\gamma(\phi(h,x,u))-V^\gamma(x)) } \\
    %= & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}
    %{\frac{1}{h}\Big(\int_0^{\infty} \|T_t \phi(h,x,u)\|_X^2 dt - V^\gamma(x) \Big) } \\
    = & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}
    \frac{1}{h}\Big( V^\gamma \Big(T_h x + \int_0^h{T_{h-s} B u(s)ds}\Big) - V^\gamma(x) \Big)  \\
%    & \quad -\int_0^{\infty} \|T_t x\|_X^2 dt \Big)  \\
    \leq & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}
    \frac{1}{h}\Big( V^\gamma \big(T_h x\big) + V^\gamma
    \Big(\int_0^h{T_{h-s} B u(s)ds}\Big) - V^\gamma(x) \Big)\\
 %& \quad \quad - V^\gamma(x) \Big)  \\
    \leq & \mathop{\overline{\lim}} \limits_{h \rightarrow +0}
    \frac{1}{h}\Big( (e^{-\gamma h} -1 ) V^\gamma(x) + V^\gamma
    \Big(\int_0^h{T_{h-s} B u(s)ds}\Big)  \Big)    \\
 \leq &  - \gamma \ V^\gamma(x) + V^\gamma (Bu(0)) \,.
    \end{align*}
}		
In the last inequality we have used the continuity of $V^\gamma$.
This shows $V^\gamma$ is an ISS-Lyapunov function (in dissipative form) and that
\eqref{eq:dissipation2} holds. Choosing a suitable Lyapunov gain $\chi \in\Kinf$, one can show that \eqref{DissipationIneq} holds and thus $V^{\gamma}$ is an ISS Lyapunov function in implication form. Coercivity is evident by construction.
\end{proof}

%%%%%%%




Finally, we can state the main result of this section:
\begin{theorem}
Let $B \in L(U,X)$. The following statements are equivalent:
\begin{enumerate}
    \item[(i)] \eqref{LinSys} is ISS.
    \item[(ii)] \eqref{LinSys} is 0-UGAS.
    \item[(iii)] $\{T_t\}_{t\geq 0}$ is an exponentially stable semigroup.
    \item[(iv)] $V$ defined in \eqref{eq:LF_LinSys_Banach} is a (not
          necessarily coercive) locally Lipschitz continuous 
%on bounded balls 
ISS Lyapunov function for \eqref{LinSys}.
%    \item [(iv b)]: There exists a noncoercive ISS Lyapunov function in the sense of Definition 4. 
    \item[(v)] $V^\gamma$ defined in \eqref{eq:eqnorm} is a coercive globally Lipschitz continuous ISS Lyapunov function for \eqref{LinSys}.
\end{enumerate}
\end{theorem}

\begin{proof}
Equivalence of the items (i) and (ii) can be derived from the variation of constants formula. The implications (ii) $\Rightarrow$ (iii) $\Rightarrow$ (iv) follow from Proposition~\ref{ConverseLyapunovTheorem_LinearSystems}.
Item (iv) implies (iii) due to Datko's Lemma, see \cite[Lemma 5.1.2,
Theorem 5.1.3, p. 215]{CuZ95}. The implication (iii) $\Rightarrow$ (ii) is clear.
(ii) implies (v) due to Proposition~\ref{p:Lyapunovfunction2} and (v) implies (i) by Proposition~\ref{Direct_LT_ISS_maxType}.
\end{proof}


\section{Remarks on non-coercivity of Lyapunov functions and admissibility of input operators}
\label{sec:Non-coercivity_and_admissibility}

In this paper, our prime interest was in "coercive" converse Lyapunov theorems. In particular, Theorem~\ref{ISS_Converse_Lyapunov_Theorem} shows that ISS is equivalent to the existence of a Lipschitz continuous \textit{coercive ISS Lyapunov function}. However, since in some cases it may be hard to construct a coercive Lyapunov function, it is strongly desirable to have criteria of ISS in terms of \textit{non-coercive ISS Lyapunov functions}. In \cite[Theorem 9]{MiW18b} it was shown that for a certain subclass of nonlinear systems 
\eqref{InfiniteDim} already the existence of a non-coercive ISS Lyapunov function is sufficient for ISS.
This was generalized to a more general class of control systems in \cite{JMP18}.
Converse non-coercive ISS Lyapunov theorems have not been studied in the literature yet.
However, for systems of the form \eqref{eq:Modified_InfDimSys_With_Disturbances} it was shown that existence of a non-coercive Lyapunov function is equivalent to a so-called integral uniform global asymptotic stability property (which is a weaker property than UGAS) \cite{MiW18a}. 

Other challenging open problems are direct and converse ISS Lyapunov
theorems for linear systems \eqref{LinSys} with admissible operators
$B$. In contrast to the case of $B\in L(U,X)$, studied in
Section~\ref{sec:LinSys}, the stability analysis of \eqref{LinSys} with an unbounded admissible operator $B$ is much more complex. 
In particular, it is not completely clear for which classes of systems \eqref{LinSys} the existence of a non-coercive Lyapunov function implies ISS. This holds e.g. if $A$ generates an analytic semigroup and the corresponding $H^{\infty}$-calculus is bounded, see \cite{JMP18} (which uses the tools from \cite{MiW18b,JSZ17}). 
On the other hand, even for such a simple ISS system as a heat equation
with Dirichlet boundary input there are no constructions of coercive
Lyapunov functions
\ifSCL{,}%
\else{}(it is not even known whether a coercive ISS Lyapunov function
exists), 
\fi{}%
but at the same time there is a construction of a non-coercive ISS Lyapunov function for this system \cite{JMP18}. 
As we have seen in Section~\ref{sec:LinSys}, an ISS Lyapunov function
(both non-coercive and coercive) for a linear system with $B\in L(U,X)$
can be chosen independently on $B$. This is not the case for systems with
unbounded admissible operators.
\ifSCL{}%
\else{}In particular, ISS Lyapunov functions showing ISS for any bounded
input operator do not have to be ISS Lyapunov functions for a given
admissible operator $B$, even if the system is actually ISS. 
\fi{}%
For some results in this direction a reader may consult \cite{JMP18}. 











\section{Admissibility of operators for linear systems}



Let $X$ be the state space, and $U$ the space of input values. And let both of them be Banach spaces.

Consider a linear system
\begin{equation}
\label{LinSys}
\begin{array}{l}
{\dot{x}=Ax+Bu,} \\
x(0)=x_0,
\end{array}
\end{equation}
where $x(t):X \to X$, $u(t):\R_+ \to U$, $A:D(A) \to X$ is a generator of $C_0$-semigroup $T(\cdot)$ on $X$ and $B:D(B) \to X$ is an input operator.

The solution of the above system is given by
\begin{equation}
\label{LinEq_IntegralForm}
x(t)=T(t)x_0 + \int_0^t{T(t-r)B u(r)dr},
\end{equation}


Let $\beta \in \rho(A)$, the resolvent set of $A$. Define $X_1$ as $D(A)$ with a norm 
\[
\|x\|_1:=\|(\beta I-A)x\|,
\]
and the space $X_{-1}$ to be completion of $X$ with respect to the norm
\[
\|x\|_{-1}:=\|(\beta I-A)^{-1}x\|.
\]

We need the following definitions

\begin{definition}
Let $U,X$ be Banach spaces and let $p \in [1,\infty]$ be given. Let also $B \in L(U,X_{-1})$. Then $B$ is called $p$-admissible \cite{TuW09}, \cite{JaP04}, \cite{Wei89b} if
\begin{equation}
\label{admissible}
 \left\| \int_0^t T(s)Bu(s)\,ds\right\|_X \le h_t \Big(\int_0^t \|u(s)\|^p_U ds \Big)^{1/p},
\end{equation}
holds for all $u \in L_{p, loc}(\R_+,U)$, all $t \geq 0$ and some constant $h_t>0$ dependent on $t$. 

If $h$ does not depend on $t$, then $B$ is called infinite-time $p$-admissible operator.
\end{definition}

Analogously, one can define $\infty$-admissible operators
\begin{definition}
Let $U,X$ be Banach spaces and let $p \in [1,\infty]$ be given. Let also $B \in L(U,X_{-1})$. The control operator $B$ is $\infty$-admissible, if
\begin{equation}
\label{infty_admissible}
 \left\| \int_0^t T(s)Bu(s)\,ds\right\|_X \le h_t \sup_{s \in[0,t]} \|u(s)\|_U,\quad  p \ge 1
\end{equation}
holds for all $u \in L_{\infty, loc}(\R_+,U)$, all $t \geq 0$ and some constant $h_t>0$ dependent on $t$. 

If $h$ does not depend on $t$, then $B$ is called infinite-time $\infty$-admissible operator.
\end{definition}


We assume without loss of generality that $h(\cdot)$ is a nondecreasing function.

\begin{lemma}
\label{GrabowskiLemma}
Let $T$ be an exponentially stable semigroup and let $p \in [1,\infty]$. Then $B$ is $p$-admissible control operator iff it is infinite-time $p$-admissible control operator.
\end{lemma}

\begin{proof}
Let $p < \infty$ (the argument is analogous for $p = \infty$). 
We mimic a proof from \cite[Lemma 1.1]{Gra95}.


Clearly, infinite-time $p$-admissibility implies $p$-admissibility.
Assume that $B$ is infinite-time $p$-admissible and pick arbitrary $\tau>0$.
Consider any $t=k\tau+t'$ for some $k \in \N$ and $t'<\tau$.
\begin{eqnarray*}
 \left\| \int_0^t T(s)Bu(s)\,ds\right\|_X  &= & \left\| \int_{k\tau}^{t\tau+t'} T(s)Bu(s)\,ds +  \sum_{i=0}^{k-1} \int_{i \tau}^{(i+1) \tau} T(s)Bu(s)\,ds\right\|_X \\
&\leq & \left\| \int_{0}^{t'} T(s+k\tau)Bu(s+k\tau)\,ds \right\|_X +  \left\| \sum_{i=0}^{k-1} \int_{0}^{\tau} T(s+i\tau)Bu(s+i\tau)\,ds\right\|_X \\
&\leq &  \|T(k\tau)\| \left\| \int_{0}^{t'} T(s)Bu(s+k\tau)\,ds \right\|_X +  \sum_{i=0}^{k-1} \|T(i\tau)\| \left\|\int_{0}^{\tau} T(s)Bu(s+i\tau)\,ds\right\|_X \\
&\leq &  Me^{-\lambda k\tau} h(t') \Big( \int_0^{t'} \|u(s + k\tau)\|^p_U ds \Big)^{1/p}  +  \sum_{i=0}^{k-1} Me^{-\lambda i\tau} 
h(\tau) \Big(\int_0^{\tau} \|u(s + i\tau)\|^p_U ds \Big)^{1/p} \\
&\leq &  Me^{-\lambda k\tau} h(\tau) \Big(\int_0^{t} \|u(s)\|^p_U ds \Big)^{1/p} +  \sum_{i=0}^{k-1} Me^{-\lambda i\tau} h(\tau) \Big(\int_0^{t} \|u(s)\|^p_U ds \Big)^{1/p} \\
&\leq &  \sum_{i=0}^{k} Me^{-\lambda i\tau} h(\tau) \Big(\int_0^{t} \|u(s)\|^p_U ds\Big)^{1/p} \\
&\leq &  \sum_{i=0}^{\infty} Me^{-\lambda i\tau} h(\tau) \Big(\int_0^{t} \|u(s)\|^p_U ds\Big)^{1/p}.
\end{eqnarray*}
Taking $h:=M h(\tau) \sum_{i=0}^{\infty} e^{-\lambda i\tau}$, we get the result.
\end{proof}

Now we have:
\begin{proposition}
\label{HauptLinSatz}
For any $p \in [1,\infty]$ the following notions are equivalent for systems \eqref{LinSys}:
\begin{enumerate}
	\item ISS w.r.t. $L_p(\R_+,U)$
	\item exponential ISS w.r.t. $L_p(\R_+,U)$
	\item 0-UGAS + infinite-time $p$-admissibility of $B$.	
	\item 0-UGAS + $p$-admissibility of $B$
\end{enumerate}
\end{proposition}

\begin{proof}
The equivalence between 1. and 2. is due to linearity of the system and can be easily verified, as in \cite[Lemma 1]{DaM13}.
The equivalence between 2. and 4. follows by considering $u \equiv 0$ and $\phi_0 \equiv 0$.
The equivalence between 3. and 4. is due to Lemma~\ref{GrabowskiLemma}.
\end{proof}

Immediately we have a corollary 
\begin{corollary}
If \eqref{LinSys} is ISS w.r.t. $L_p(\R_+,U)$, then \eqref{LinSys} is ISS w.r.t. $L_q(\R_+,U)$ for all $q \geq p$.
In particular, \eqref{LinSys} is ISS.
\end{corollary}

\begin{proof}
H\"older inequality implies that $p$-admissibility implies $q$-admissibility for $p \leq q$. 
\end{proof}







\begin{definition}
We call a semigroup $T$ uniformly bounded, if $ \exists M$: $\|T(t)\| \leq M$ for all $t$.
\end{definition}

\begin{remark}
\label{StrongStability_UnifBoundedness}
If $T$ is a strongly stable semigroup, then it is also uniformly bounded.
Indeed, since $T$ is strongly stable, then $\forall x \in X$ $\sup_{t \geq 0} \|T(t)x\|_X < \infty$, and by Banach-Steinhaus theorem $\sup_{t \geq 0}\|T(t)\| < \infty$.
\end{remark}


Now we introduce a weaker ISS notion
\begin{definition}
\eqref{LinSys} is called weakly input-to-state stable (wISS) w.r.t. input space $U_c$, if it is 0-GAS and there exist $\gamma \in \Kinf$ 
so that the following estimate holds:
\begin{equation}
\label{wISS_Estimate}
\|\phi(t,\phi_0,u)\|_X \leq \|T(t)\phi_0\|_X + \gamma(\|u\|_{U_c}), \quad \forall \phi_0 \in X,\ \forall u, \ \forall t \geq 0.
\end{equation}
\end{definition}

Analogously we have the following criterion
\begin{proposition}
\label{HauptLinSatz_weakISS}
For any $p \in [1,\infty]$ the following notions are equivalent:
\begin{enumerate}
	\item wISS w.r.t. $L_p(\R_+,U)$
	\item 0-GAS + infinite-time $p$-admissibility of $B$.
	\item strong stability of $T(\cdot)$ + infinite-time $p$-admissibility of $B$.
\end{enumerate}
\end{proposition}

\begin{proof}
The equivalence between 1. and 3. follows by considering $u \equiv 0$ and $\phi_0 \equiv 0$.
And $0$-GAS is equivalent to strong stability of $T(\cdot)$ due to Remark~\ref{StrongStability_UnifBoundedness}.
\end{proof}




\subsection{Other}

In what follows we are going to define a weaker notion of ISS. First we need several additional stability notions.
\begin{definition}
\eqref{LinSys} is called Lyapunov stable if  $\forall \eps >0$ $\exists$ $\delta$: $\forall x_0 \in X: \|x_0\|_X < \delta$
it follows $\|T(t)x_0\|_X < \eps$.
\end{definition}

\begin{definition}
\eqref{LinSys} is called globally asymptotically stable at zero (0-GAS), if for $u \equiv 0$ it is Lyapunov stable and globally attractive.
\end{definition}

\begin{definition}
We call a semigroup $T$ uniformly bounded, if $ \exists M$: $\|T(t)\| \leq M$ for all $t$.
\end{definition}


\begin{proposition}
\eqref{LinSys} is 0-GAS iff $A$ generates a strongly stable semigroup $T$.
\end{proposition}

\begin{proof}
If \eqref{LinSys} is 0-GAS, then it is 0-GATT, which implies strong stability of the semigroup $T$.
According to Remark~\ref{StrongStability_UnifBoundedness}, if $T$ is strongly stable, then it is uniformly bounded, which implies Lyapunov stability of \eqref{LinSys}.
Since strong stability of $T$ implies 0-GATT of \eqref{LinSys}, the claim is proved.
%Now let \eqref{LinSys} be Lyapunov stable. Pick any $\eps>0$. Then there exist $\delta>0$: $\forall x_0: \|x_0\|=\delta$ holds
%\[
%\|T(t)x_0\| <\eps= \frac{\eps}{\delta}\|x_0\|. 
%\]
%Due to linearity of $T(t)$ the above inequality holds for all $x_0\in X$ and hence $\|T(t)\| \leq \frac{\eps}{\delta}$. 
\end{proof}

%Denote by $\rho(A)$ the spectral radius of an operator $A$.
%\begin{proposition}
%If $T$ is uniformly bounded, then $\rho(T(t)) \leq 1$ for all $t$.
%\end{proposition}
%
%\begin{proof}
%$\rho(T(t))=\lim_{n \to \infty}\|(T(t))^n\|^{\frac{1}{n}}= \lim_{n \to \infty}\|T(nt)\|^{\frac{1}{n}} \leq \lim_{n \to \infty}M^{\frac{1}{n}}=1.$
%\end{proof}


\begin{definition}
\eqref{LinSys} is called weakly input-to-state stable (wISS) w.r.t. input space $U_c$, if it is 0-GAS and there exist $\gamma \in \Kinf$ 
so that the following estimate holds:
\begin{equation}
\label{wISS_Estimate}
\|\phi(t,\phi_0,u)\|_X \leq \|T(t)\phi_0\|_X + \gamma(\|u\|_{U_c}), \quad \forall \phi_0 \in X,\ \forall u, \ \forall t \geq 0.
\end{equation}
\end{definition}

\begin{proposition}
\label{wISS_L1_space}
\eqref{LinSys} is ISS w.r.t $U_c=L_1(\R_+,\R^m)$ iff it is 0-GAS. 
\end{proposition}

\begin{proof}
Let \eqref{LinSys} be 0-GAS. Then $T$ is uniformly bounded semigroup, and thus
\begin{eqnarray}
\label{weak_iISS}
\|s(t)\|_X  & \leq & \|T(t)s_0\|_X + \int_0^t{\|T(t-r)\|\|B\| \|u(r)\|_U dr}, \notag \\
& \leq & \|T(t)s_0\|_X + M \|B\| \int_0^t{\|u(r)\|_U dr}
\end{eqnarray}
\end{proof}


\subsection{Bounded input operators}

Let us consider a special case when $B\in L(U,X)$. Since bounded operators are automatically $p$-admissible for all $p \in [1,\infty]$, the results simplify greatly.


Figure~\ref{LinSys_Implikationen} presents the connections between different stability properties for systems with bounded input operators.

\begin{figure}[tbh]
\centering
\begin{tikzpicture}[text width=2cm, minimum height=2em, text centered]
%\begin{tikzpicture}
%\node [circle, draw] (5em) (HARDWARE){Interfaces};

\node (UGAS)[rectangle, draw]  at (0,0) {0-UGAS};
\node (ISS)[rectangle, draw, text width =2cm, text centered]  at (3,0) {ISS w.r.t. $L_{\infty}$};

\node (wISS)[rectangle, draw]  at (6,-1.5) {wISS};

\node (GAS)[rectangle, draw]  at (0,-3) {0-GAS};

\node (LpISS)[rectangle, draw, text width =2cm, text centered]  at (6,0) {ISS w.r.t. $L_{p}$};
\node (iISS)[rectangle, draw]  at (9,0) {iISS};

%\node (iISS)[rectangle, draw]  at (6,0) {iISS};
\node (wiISS)[rectangle, draw]  at (6,-3) {wISS w.r.t. $L_1$};
\node (T_exp)[rectangle, draw]  at (-3.5,0) {$T$ is exp stable};

%\node (T_st_ub)[rectangle, draw]  at (-5,-3) {$T$ is strongly stable};

%\node (T_ub)[rectangle, draw]  at (-3.5,-3) {$T$ is uniformly bounded};
\node (T_st)[rectangle, draw]  at (-3.5,-3) {$T$ is strongly stable};
%\node (BadBym3) at (-3.5,-3.5)  {$\Downarrow$};

%\node (BadBym3) at (-3,-4)  {$?\Rightarrow$};

\node (BadBym) at (0.3,-1.5)  {$\not\Uparrow$};
\node (BadBym2) at (6,-2.15)  {$\not\Uparrow$};

%\node (BadBym3) at (3.8,-0.8)  {?$\nwarrow$};

 \draw[thick,double,<->] (ISS) to (UGAS);
 \draw[thick,double,<->] (ISS) to (LpISS);
 \draw[thick,double,<->] (LpISS) to (iISS);
 \draw[thick,double,<->] (T_exp) to (UGAS);

 \draw[thick,double,->] (ISS) to (wISS);
 
\draw[thick,double,->] (UGAS) to (GAS);
%\draw[thick,double,->] (UGAS) to (GAS);

\draw[thick,double,<->] (wiISS) to (GAS);
\draw[thick,double,<->] (T_st) to (GAS);

\end{tikzpicture}
\caption{Connections between stability properties for linear systems with bounded input operators \eqref{LinSys}}
\label{LinSys_Implikationen}
\end{figure}



\textcolor{red}{Some considerations about wISS.}

Consider \eqref{LinSys} with constant in time inputs. For all $u \in U$ define $\tilde{u}=\frac{u}{\|u\|}$.

Then solution of \eqref{LinSys}, corresponding to $s_0=0$ and $u \equiv const$ can be estimated as
\begin{eqnarray*}
\|s(t)\|_X = \left\| \int_0^t{T(t-r) B \tilde{u} dr} \right\| \|u\|_U = \left\| \int_0^t{T(r) B \tilde{u} dr} \right\| \|u\|_U,
\end{eqnarray*}
I think, that the gain can in the definition of wISS can be chosen linear without any restrictions, and this implies that there exists $M>0$
\[
\left\| \int_0^t{T(r) B \tilde{u} dr} \right\| \leq M \quad \forall \tilde{u} \in U, \|\tilde{u}\|_U=1, \forall t \geq 0. .
\]
If $B$ is invertible operator, then it is the same as 
\[
\left\| \int_0^t{T(r) x dr} \right\|  \leq M \quad \forall x \in X, \|x\|_X=1, \forall t \geq 0..
\]
Compare to the Datko's Lemma, which tells that $T$ is exponentially stable iff there exists $M>0$:
\[
 \int_0^t{\|T(r) x\|^2 dr} \leq  M \quad \forall x \in X, \forall t \geq 0.
\]

Also note, that if for some $t_0$ $\|T(t_0)\|<1$, then $T$ is exponentially stable. But if $T$ is exponentially stable, then the system \eqref{LinSys} is ISS. Thus, if there is a gap between ISS and wISS, then it is for semigroups $T$ with $\|T(t)\| \geq 1$ for all $T$.




We define another notion, involving integral estimates of an input and which corresponds to integral ISS as 0-GAS corresponds to 0-UGAS$x$.
\begin{definition}
\eqref{LinSys} is called weakly integral input-to-state stable (iISS) iff it is 0-GAS and there exist $\alpha, \gamma \in \Kinf$ so that
\begin{equation}
\label{wiISS_Estimate}
\alpha(\|\phi(t,\phi_0,u)\|_X) \leq \|T(t)\phi_0\|_X + \int_0^t \gamma(\|u(s)\|_U)ds, \quad \forall \phi_0 \in X,\ \forall u, \ \forall t \geq 0.
\end{equation}
\end{definition}

From Proposition~\ref{wISS_L1_space} it follows (by taking $\alpha := id$ and $\gamma := c \cdot id$ for large enough $c>0$):
\begin{corollary}
The system \eqref{LinSys} is wISS w.r.t $L_1([0,\infty),U)$ iff it is weakly integral ISS.
\end{corollary}



\textcolor{red}{Essentially for small-gain results the function $\beta$, which describes the transient behavior of the system, doesn't play an important role. On the contrary, the gains are essential. Since the weak formulation of integral ISS and ISS properties differs only in the transient term, it seems to be interesting to check, whether the study of interconnections of such "weak" systems is as prolific, as is the interconnection theory of standard ISS/iISS theory?}








\section{Discussion with Felix}


\begin{theorem}
\label{thm:Gen_ISS_LF_Construction-Discussion}
Let $A$ be  the generator of a $C_0$-semigroup $(T(t))_{t\ge 0}$ on a Hilbert space $X$.

Assume that there is an operator $P\in L(X)$ satisfying the following conditions:
\begin{itemize}
	\item[(i)] \label{item:Gen_Converse_Lyap_Theorem_1} $P$ satisfies
\begin{eqnarray}
\re\scalp{Px}{x}_X > 0,\quad x\in X\backslash\{0\}.
\label{eq:Positivity}
\end{eqnarray}
	\item[(ii)] \label{item:Gen_Converse_Lyap_Theorem_2} $P$ satisfies Lyapunov inequality 
%\begin{eqnarray}
%\scalp{Ax}{Px}_X + \scalp{Px}{Ax}_X  \leq  -\scalp{x}{x}_X,\quad x\in D(A),
%\label{eq:LyapIneq}
%\end{eqnarray}
\begin{eqnarray}
\re\scalp{(PA+A^*P)x}{x}_X \leq  -\scalp{x}{x}_X,\quad x\in D(A),
\label{eq:LyapIneq}
\end{eqnarray}
		\item[(iii)] \label{item:Gen_Converse_Lyap_Theorem_3} It holds that $Im(P) \subset D(A^*)$.
		%\item[(iv)] \label{item:Gen_Converse_Lyap_Theorem_4} either $P=P^*$, or $PA$ is bounded
		\item[(iv)] \label{item:Gen_Converse_Lyap_Theorem_4} $PA$ is bounded.
\end{itemize}
%\begin{eqnarray}
%\re\scalp{(PA+A^\ast P)x}{x}_X \leq -\|x\|^2_X,\quad x\in D(A).
%\label{eq:Gn_Lyap_Ineq}
%\end{eqnarray}
Then
\begin{equation}
\label{Lyap}
 V(x) := \re\, \langle Px,x\rangle_X
 \end{equation}
is a non-coercive ISS Lyapunov function for \eqref{InfiniteDim2}
with any $\infty$-admissible input operator $B\in L(U,X_{-1})$,
satisfying for each $\eps>0$ the dissipative inequality
\begin{align}
\label{ex:Dissipative_Inequality_linear_system}
 \dot{V}_u(x_0) \le&  (\varepsilon-1) \|x_0\|_X^2 + c(\eps) \|u\|^2_\infty,
%\le&  -\|x_0\|^2  + ( 2\|A_{-1}^{-1}B\|^2   + \| A_{-1}^{-1}B\|\kappa(0))  \| u(0)\|^2.
\end{align}
where 
\begin{align*}
c(\eps):=& \frac{1}{4\varepsilon}(\|A^\ast P\|_{L(X)} +\|PA\|_{L(X)})^2 \|A^{-1}_{-1}B\|_{L(U,X)}^2M^2\\
&\qquad\qquad\qquad+ M\|A^\ast P\|_{L(X)} \| A_{-1}^{-1}B\|_{L(U,X)}  \kappa(0).
\end{align*}
and
$\kappa(0)=\lim_{t \searrow 0}\kappa(t)$, where $\kappa(t)>0$ satisfies
\[ \left\|\int_0^t T_{-1}(t-s)Bu(s)\, ds\right\|_X \le \kappa(t) \|u\|_{\infty}, \qquad u\in L^\infty([0,t),U).\]
%\begin{align*}
%\dot{V}_u(x) &\le- (1-\delta -\varepsilon ) \|x_0\|_X^2\\
%& +\left( \frac{(\|A^\ast A^{-1}\|_{L(X)} +1)^2 \|A^{-1}_{-1}B\|^2}{4\varepsilon}+ \| A_{-1}^{-1}B\|  \kappa(0)\right) \|u\|^2_{\infty}
%%\label{eq:}
%\end{align*}
%for $\varepsilon\in (0, 1-\delta) $, $x_0\in X$ and $u\in L^\infty([0,\infty),U)$.
In particular, \eqref{InfiniteDim2} is ISS for such $B$.
\end{theorem}


\vspace{15mm}

Consider a linear system with the generator $A:=\tilde{A} - cI$, where 
$\tilde{A}^* = -\tilde{A}$ and $c>0$.
Clearly, $\sigma(A) \subset i\R  -c$.
Furthermore, $A$ generates a strongly continuous semigroup. We would like to use Theorem~\ref{thm:Gen_ISS_LF_Construction-Discussion}
in order to show that \eqref{Lyap} with $P:=-A^{-1}$ defines an ISS Lyapunov function 
\begin{eqnarray}
V(x) := \re \scalp{-A^{-1}x}{x}.
\label{eq:LyapFun_Skewadjoint_case}
\end{eqnarray}
for any $\infty$-admissible operator $B$. 

Clearly, $P\in L(X)$.
Furthermore, $PA = -I \in L(X)$ and
\begin{eqnarray}
Im(P) = Im(A^{-1}) = D(A) = D(\tilde{A})= D(\tilde{A}^*) = D((\tilde{A}-cI)^*) = D(A^*).
\label{eq:ImageEmbedding}
\end{eqnarray}
Furthermore, it holds that
\begin{eqnarray}
\re\scalp{(PA+A^*P)x}{x}_X  
&=& \re\scalp{(-I+(\tilde{A}-cI)^*(-A^{-1}))x}{x}_X \nonumber\\
&=& \re\scalp{(-I+(-\tilde{A}-cI)(-A^{-1}))x}{x}_X \nonumber\\
&=& \re\scalp{(-I+(-A-2cI)(-A^{-1}))x}{x}_X \nonumber\\
&=& \re\scalp{2c A^{-1}x}{x}_X \nonumber\\
&=& -2c V(x).
\label{eq:Lyapunov_Equation_SkewAdjoint}
\end{eqnarray}

The operator $-A^{-1}=-(\tilde{A} - cI)^{-1}$ is a diagonal operator with the eigenvalues $s_k:=-\frac{1}{-c+i\lambda_k}$, where $i\lambda_k$, $k\in\N$ are the eigenvalues of the operator $\tilde{A}$.
Clearly,
\[
s_k = -\frac{-c-i\lambda_k}{c^2+\lambda_k^2}= \frac{c}{c^2+\lambda_k^2} + \frac{\lambda_k}{c^2+\lambda_k^2}. 
\]
Assume that $X$ is a separable Hilbert space and let $\{e_i\}_{i\in\N}$ be an orthogonal basis in $X$.
Then for each $x\in X$ it holds that $x = \sum_{i=1}^\infty x_i e_i$.
So as I understand, by this spectral decomposition we obtain that $V$ is not coercive.

This leads to problems, as \eqref{eq:Lyapunov_Equation_SkewAdjoint}, which is the derivative of $V$ for $u\equiv 0$
is not a 'real' non-coercive Lyapunov function and without further analysis such a function even does not guarantee 
0-UGAS of a system, see \cite[Example 6.2]{MiW17a}.

May be for diagonal operators this Lyapunov function will be still OK, because the counterexample in  \cite[Example 6.2]{MiW17a} was for the systems with large Jordan blocks. 

\begin{remark}
\label{rem:} 
Actually, we obtain 0-UGAS of the system with this $A$ by using $P:=I$, but this will not work for ISS analysis with the theorem which we have.
\end{remark}


\subsection{Questions}


\begin{itemize}
	\item How to construct an ISS Lyapunov function for $A:=\tilde{A} - cI$, where 
$\tilde{A}^* = -\tilde{A}$ and $c>0$?
	\item Actually, the real problem will be to obtain an ISS Lyapunov functions for hyperbolic boundary control systems with the dissipation at the boundary. 
	To have such a construction and to compare it with the construction of Lyapunov functions for analytic systems would be a strong result.
	
	\item How to use the information about the grade of admissibility of the operator $B$ in the construction of the ISS Lyapunov functions.
In particular, assume that $A$ generates an analytic semigroup. Then fractional powers of an operator $A$ can be defined via Cauchy integral.
Assume that $B$ is $p$-admissible with $p<\infty$.
	
	Can we consider Lyapunov functions of the form
\[
V(x) = -\re\scalp{A^{-1+\eps}x}{x},\quad x\in X
\]
where $\varepsilon>0$ depends on $p$?

Does it hold then that $A^{-1+\varepsilon}B$ is bounded for a certain $\varepsilon>0$?

In particular, can we use this Lyapunov function for $2$-admissible operators with $\varepsilon=\frac{1}{2}$?
 
	\item Idea of Felix to use $A^{-1/2}$ in combination with the construction of coercive ISS Lyapunov functions for systems with bounded operators.
	
	\item Positive systems: getting the results from MKK paper for the general class of positive systems, possibly also for nonlinear (at least semilinear) ones.
	\item Can we use the general result on construction of Lyapunov functions for systems with admissible operators for some other cases than $P:=A^{-1}$? 
	One should try $P:=P_1A^{-1}$, where $P_1$ is a bounded operator.
Maybe with $P_1$ positive and self-adjoint or maybe skew-adjoint?
\end{itemize}



\subsection{Well known example: Transport equation with a boundary input}

Consider a transport equation 
\begin{eqnarray}
\frac{\partial x}{\partial t}(t,z) + \frac{\partial x}{\partial z}(t,z) =0, \quad (t,z) \in (0,+\infty) \times (0,1)
\label{eq:TransportEquation}
\end{eqnarray}
subject to a boundary condition
\begin{eqnarray}
x(t,0)=u(t)
\label{eq:TransportEquation_Dirichlet_BC}
\end{eqnarray}
and an initial condition
\begin{eqnarray}
x(0,z)=x_0(z),\quad z\in(0,1).
\label{eq:TransportEquation_Dirichlet_Init_Cond}
\end{eqnarray}

\begin{proposition}
\label{prop:Transport_Equation_eISS} 
Let $X:=L_2(0,1)$ and $\Uc:=PC(\R_+,\R)$. Then the system \eqref{eq:TransportEquation}, \eqref{eq:TransportEquation_Dirichlet_BC}, \eqref{eq:TransportEquation_Dirichlet_Init_Cond} is exponentially ISS.
\end{proposition}

\begin{proof}
Pick any $\mu>0$. Choose the following ISS Lyapunov function candidate: 
\[
V(x):=\int_0^1 e^{-\mu z}x^2(z)dz.
\]
Clearly, $V$ is coercive as
\begin{eqnarray}
e^{-\mu} \|x\|^2_X \leq V(x) \leq \|x\|^2_X \quad x\in X.
\label{eq:Coercive_Estimate_Transport_LF}
\end{eqnarray}
Let us compute the Lie derivative for $V$ along \eqref{eq:TransportEquation} with boundary conditions \eqref{eq:TransportEquation_Dirichlet_BC}. We would like to show this first for classical solutions, as in this simplifies the computation of the Lie derivative of $V$ considerably. 

%{\color{red}
%Actually, for which initial conditions the classical solution exists?
%}

Assume that $x\in C^1(0,1)$ and $u\in C^1(\R)$. For these initial conditions and boundary inputs the corresponding classical solution of  \eqref{eq:TransportEquation}, \eqref{eq:TransportEquation_Dirichlet_BC} exists.

Then
\begin{eqnarray*}
\dot{V}(x) &=& \int_0^1e^{\mu z} \frac{d}{dt}(x^2(z))dz\\
&=& \int_0^1e^{\mu z}  2x(z)\frac{\partial x}{\partial t}(z)dz\\
\big[x \mbox{ is a classical solution of \eqref{eq:TransportEquation}}\big] &=& -\int_0^1e^{-\mu z} 2x(z)\frac{\partial x}{\partial z}(z)dz\\
&=& -\int_0^1e^{-\mu z} 2x(z)\frac{\partial x}{\partial z}(z)dz\\
&=& -e^{-\mu z}x^2(z)\Big|_{z=0}^1 -\mu  \int_0^1e^{-\mu z} x^2(z)dz\\
&=& -e^{-\mu }x^2(1) + x^2(0)  -\mu  \int_0^1e^{-\mu z} x^2(z)dz\\
&\leq& x^2(0)  -\mu  \int_0^1e^{-\mu z} x^2(z)dz\\
&\leq& \|u\|_\Uc^2  -\mu  V(x),
\end{eqnarray*}
which shows that $V$ is an ISS Lyapunov function for \eqref{eq:TransportEquation} with boundary inputs \eqref{eq:TransportEquation_Dirichlet_BC} on the space $C^1(0,1)$, for which the above computations are valid.

As $C^1(0,1)$ is dense in $L^2(0,1)$ 
%by Propositions~\ref{prop:Cp_is_dense_in_C} and \ref{prop:Dense_subsets_of_Lp}, 
we may use the density argument (Lemma~\ref{lem:Density_Arg_eISS}).

%to show that the system \eqref{eq:TransportEquation}, \eqref{eq:TransportEquation_Dirichlet_BC}
%is ISS over the whole state space $L^2(0,1)$.

%{\color{red} We need to show that Assumption~\ref{ass:Continuous_Dependense_Density_Argument} 
%holds. 
%}

Now Theorem~\ref{thm:eISS_LF_with_good_psi_implies_eISS} implies that \eqref{eq:TransportEquation}, \eqref{eq:TransportEquation_Dirichlet_BC}, \eqref{eq:TransportEquation_Dirichlet_Init_Cond} is exponentially ISS.
\end{proof}

\begin{remark}
\label{rem:More_General_1d_Systems} 
Much more general class of hyperbolic first order systems over a 1-dimensional spatial domain are considered by means of a Lyapunov method in \cite{TPT16}.
\end{remark}


%Thinking about analytic semigroups, we can understand the non-coercivity in a Lyapunov function as a way to imbed very nice spectral properties
%(real negative spectrum, unbounded to the left) into the Lyapunov function, which makes possible then to use this information for certain other purposes.





{\color{blue}



\subsection{JMP Paper: Further questions}

Possible further problems for this paper:
\begin{itemize}
	\item Can we use the derived Lyapunov function for the systems with additional nonlinearity, which can be quite nice?

	\item Coupling a linear PDE via boundary with a nonlinear ODE. 
	First constructing noncoercive ISS LFs, and use non-coercive small-gain theorem to construct a non-coercive LF for the whole system, and then use the direct non-coercive ISS Lyapunov theorems to establish ISS of the whole system

	\item Is integral-to-integral ISS equivalent to the following property:

there are $\alpha\in\K$ and $\beta\in \KL$, $\sigma\in\Kinf$ so that
for all $x\in X$, $u\in\Uc$ and $t\geq 0$ it holds that
\begin{eqnarray*}
%\label{eq:ii-ISS}
\int_t^\infty \alpha(\|\phi(s,x,u)\|_X) ds \leq \beta(\|x\|_X,t) + \int_t^\infty \sigma(\|u(s)\|_U)ds.
\end{eqnarray*}

	\item Does ISS imply integral-to-integral ISS? Sontag has shown this for ODEs in \cite{Son98} by means of converse ISS Lyapunov theorems. As long as such theorems work for infinite-dimensional systems, we can show the converse implications for such systems as well. But we have converse ISS Lyapunov theorems only for some subclasses of inf-dim control systems right now. Can we obtain a non-Lyapunov proof?

	\item We know that ISS $\Iff$ 0-UGAS $\wedge$ $\infty$-admissibility of $B$.
	
	 We know that 0-UGAS $\Iff$ there is a (positive, bounded, self-adjoint) solution $P$ of the Lyapunov equation (or inequality).
	
	Can we characterize admissibility of an input operator $B$ by means of the properties of the operator $P$?
	
	In particular, what is the relation between boundedness of $PB$ and $\infty$-admissibility of $B$?
\end{itemize}


}



\section{Exercises}

\section{Concluding remarks}

Our exposition of Section~\ref{sec:Boundary control systems} follows \cite[Chapter 11]{JaZ12}.
Port-Hamiltonian systems, which play an important role in modeling many classes of physical systems are a special class of boundary control systems, see \cite{JaZ12} for more on this theory.



==> chap_Unsorted_material.tex <==

\chapter{Unsorted material}
\label{chap:Unsorted}

 




